The Longer the Better? The Interplay Between Review Length and Line of Argumentation in Online Consumer Reviews

Review helpfulness serves as focal point in understanding customers' purchase decision-making process on online retailer platforms. An overwhelming majority of previous works find longer reviews to be more helpful than short reviews. In this paper, we propose that longer reviews should not be assumed to be uniformly more helpful; instead, we argue that the effect depends on the line of argumentation in the review text. To test this idea, we use a large dataset of customer reviews from Amazon in combination with a state-of-the-art approach from natural language processing that allows us to study argumentation lines at sentence level. Our empirical analysis suggests that the frequency of argumentation changes moderates the effect of review length on helpfulness. Altogether, we disprove the prevailing narrative that longer reviews are uniformly perceived as more helpful. Our findings allow retailer platforms to improve their customer feedback systems and to feature more useful product reviews.

==> tex/generic/index.tex <==
\pdfbookmark[0]{\indexname}{index}
\printindex
\clearpage

==> tex/generic/lists.tex <==
%%      \pdfbookmark[0]{\listfigurename}{LOF}
  \listoffigures

%%      \pdfbookmark[0]{\listalgorithmname}{LOF}
  \listofalgorithms

%%      \pdfbookmark[0]{\listtablename}{LOT}
%  \listoftables

\clearpage


==> tex/generic/notation.tex <==
\pdfbookmark[0]{Notation}{Notation}

\chapter*{Notation}
  \label{chp:notation}
  
\begin{longtable}{ll}
%  $\exists$ & exists at least once \\
  $\forall$ & for all \\
  $\fulfill$ & shall fulfill \\

%  $\N$ & set of all integers greater than zero \\
%  $\N_0$ & set of all all integers greater than or equal to zero, \ie $\N \cup \set{0}$ \\
  $\R$ & set of all real numbers \\

  $x \in S$ & $x$ is an element of set $S$ \\
  $\intervaloo{a}{b}$ & open interval of all $x \in\R$ with $a < x < b$ \\

  $\vecval{v} \vecsize{n}$ & real vector of size $n$ \\
  $\matval{A} \matsize{n}{m}$ & real matrix of size $n \times m$ \\
  $\lambda$ & eigenvalue \\

  $\min$, $\max$ & minimum, maximum \\
  $\conj{x}$ & complex conjugate \\
  $\abs{x}$ & absolute value \\
  $\norm{\vecval{v}}$ & Euclidean norm \\
  $\vecprod{\vecval{v}}{\vecval{w}}$ & vector product defined as $\vecval{v}\transpose \vecval{w}$\\
  $\vecval{v} \inlineortho \vecval{w}$ & $\vecval{v}$ is orthogonal to $\vecval{w}$ \\

  $\unitvec{p}{n}$ & almost zero vector of size $n$ whose $p$-th entry is one  \\
  $\zerovec{n}$ & zero vector of dimension $n$ \\
  $\zeromat{n}{m}$ & zero matrix of size $n \times m$ \\
  $\identitymat{n}$ & identity matrix of size $n \times n$ \\%
%
  $\matval{A}\transpose$ & transposed matrix \\
  $\matval{A}\pseudoinverse \matsize{n}{m}$ & pseudoinverse of $\matval{A}\matsize{m}{n}$ such that $\matval{A}\pseudoinverse \matval{A} = \identitymat{n}$ \\
  $\diag{\matval{A}}$ & diagonal entries of matrix $\matval{A}$ \\
  $\concatvec{x_1, \ldots, x_n}$ & concatenated vector \\
  $\concatmat{\vecval{v}_1 \concatmatsep \ldots \concatmatsep \vecval{v}_n}$ & concatenated matrix \\
  $\lincomb{\vecval{v}_1, \ldots, \vecval{v}_n}$ & linear hull of a set of $n$ vectors \\

  $p(\matval{A})$ & polynomial in $\matval{A}$ \\

  $u_x$ & derivative of function $u$ in $x$-direction \\
  $\Laplace$ & Laplace operator \\

  $\Oh{n}$ & Landau notation for asymptotic behavior \\
  
%  $\sstep{V}_k$ & newly generated $s$-step basis vectors from iteration $k$ \\
%  $\Sstep{V}_k$ & assembled $s$-step basis vectors of  \\
%  $\dual{\Sstep{T}}$ & transposed problem $\matval{A}\transpose \Sstep{W} = \Sstep{W} \dual{\Sstep{T}}$  \\
\end{longtable}

%% F_k^{i,j} iter k, entry i,j
%% TODO: append/underline

%\begin{longtable}{ll}
%$\floor{x}$ & floor \\
%$\ceil{x}$ & ceil \\
%$\R^+$ & set of all positive real numbers \\
%$\R^{\geq c}$ & set of all real numbers greater than or equal to $c \in \R$  \\
%$\R^{m\times n}$ & real matrices of size $m \times n$ \\
%$\Re{x}$ & real part of $x$ \\
%$\Im{x}$ & imaginary part of $x$ \\
%%$\powerset{S}$ & power set of $S$, \ie $\powerset{S} = \set[X]{X \subseteq S}$ \\
%$\inf$ & infimum \\
%$\sup$ & supremum \\
%$\det{A}$ & determinant of $A$ \\
%$\sign{x}$ & sign function with $\sign{0} = 0$ \\
%$\intervalcc{a}{b}$ & closed interval $\set[x \in \R]{a \leq x \leq b}$ \\
%$\intervaloo{a}{b}$ & open interval $\set[x \in \R]{a < x < b}$ \\
%$\set{a, b}$ & the set compromising the elements $a$ and $b$  \\
%$A \subset B$ & $A$ is a real subset of $B$ \\
%$A \subseteq B$ & $A$ is a real subset of $B$ or $A$ is equal to $B$ \\
%$\left(x_n\right)_{n\in\N}$ & sequence $x_1, x_2, x_2, \ldots$ \\
%$X$ & domain of a function $f$ \\
%$f \equiv g$ & equation $f(x) = g(x)$ holds for all $x$ of the domain \\
%$x \uparrow p$ & $x$ approaches $p$, but $x < p$ for any value of $x$ \\
%$x \downarrow p$ & $x$ approaches $p$, but $x > p$ for any value of $x$ 
%\end{longtable}


==> tex/generic/toc.tex <==
    \pdfbookmark[0]{\contentsname}{TOC}

    \let\captionmathfont=\captionmathfonttoc
    \let\sectionmathfont=\sectionmathfonttoc

  \tableofcontents
  
    \let\captionmathfont=\captionmathfonttext
    \let\sectionmathfont=\sectionmathfonttext
%        \clearpage

==> tex/macros.tex <==
\input{tex/macros/maths}
\input{tex/macros/abbreviations}
\input{tex/macros/semantics}
\input{tex/macros/tables}

%\newcommand{\AusrichtungTabelle}{\sisetup{parse-numbers = false,input-symbols=()*, table-figures-integer = 4, table-figures-decimal=6, table-number-alignment=center}}
%\newcommand{\AusrichtungTabelleII}{\sisetup{parse-numbers = false,input-symbols=()*, table-figures-integer = 3, table-figures-decimal=7, table-number-alignment=center}}
%\newcommand{\AusrichtungTabelleIII}{\sisetup{parse-numbers = false,input-symbols=()*., table-figures-integer = 3, table-figures-decimal=5, table-number-alignment=center}}

==> tex/macros/abbreviations.tex <==
\newcommand\ie{i.\,e.\xspace}
\newcommand\eg{e.\,g.\xspace}
\newcommand\Eg{E.\,g.\xspace}
\newcommand\NB{N.\,B.\xspace}
\newcommand\BSc{B.\,Sc.\xspace}
\newcommand\MSc{M.\,Sc.\xspace}
\newcommand\PhD{Ph.\,D.\xspace}
\newcommand\etc{etc.\xspace}
\newcommand\etal{et\,al.\xspace}
\newcommand\page[1]{p.\,#1}
\newcommand\pages[1]{pp.\,#1}
\newcommand\US{U.\,S.\xspace}

\newcommand\zB{z.\,B.\xspace}
\newcommand\proz{\,\%\xspace}

\newcommand\thesis{thesis\xspace}

==> tex/macros/maths.tex <==
% -- Vektor fett darstellen -----------------
% \let\oldvec\vec
% \def\vec#1{{\boldsymbol{#1}}} %Fetter Vektor
% \newcommand{\ve}{\vec} %
% -------------------------------------------

\newcommand{\itemmath}[1]{$\bm{\mathsf{#1}}$}
\newcommand{\captionmath}[1]{$\protect\captionmathfont{#1}$}
  \newcommand{\captionmathfonttoc}[1]{\mathsf{#1}}
  \newcommand{\captionmathfonttext}[1]{\bm{\mathsf{#1}}}
  \let\captionmathfont=\captionmathfonttext
\newcommand{\sectionmath}[1]{$\protect\sectionmathfont{#1}$}
  \newcommand{\sectionmathfonttoc}[1]{#1}
  \newcommand{\sectionmathfonttext}[1]{\mathsf{#1}}
  \let\sectionmathfont=\sectionmathfonttext

%% from package braket
{\catcode`\|=\active
  \xdef\Concat{\protect\expandafter\noexpand\csname Concat \endcsname}
  \expandafter\gdef\csname Concat \endcsname#1{\begingroup
     \ifx\SavedDoubleVert\relax
       \let\SavedDoubleVert\|\let\|\BraDoubleVert
     \fi
     \mathcode`\|32768\let|\BraVert
     \left[{#1}\right]\endgroup}
}

\newcommand{\mathup}[1]{\mathrm{#1}}

\newcommand\eref[1]{\tag*{\ref{#1}}} % Formel erscheint erneut und soll gleiche Formelnummer wie beim ersten Auftreten erhalten

\newcommand\const{\mathrm{const}}
\newcommand\rp{^{-1}}
\newcommand\rps{^{-2}}
\newcommand\rpc{^{-3}}

\newcommand\transpose{^T} %{^\top}
\newcommand\rptranspose{^{-T}} %^{^{-\top}}
\newcommand\pseudoinverse{^{+}}

\newcommand\define{:=} % :=, \ensuremath{\mathrel{\stackrel{\mathrm{def}}{=}}}
\newcommand\ldefine{=:}
\newcommand{\setsep}{\, | \,}
%\newcommand\set[1]{\left{#1\right}}
%\newcommand\set*[2]{\left{ #1 \setsep #2 \right}}
%\newcommand{\set}[2][]{%
%    \ifthenelse{\equal{#1}{}}{\left\{ #2 \right\}}{\left\{ #1 \setsep #2 \right\}}%
%  }

\newcommand{\norm}[1]{\left\Vert #1 \right\Vert_2}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

%\newcommand{\vecval}[1]{\mathbf{#1}}
\newcommand{\vecval}[1]{{\color{MathsVectorColor}\bm{#1}}}
\newcommand{\matval}[1]{{\color{MathsMatrixColor}#1}}
  %\newcommand{\vecval}[1]{\bm{#1}}
  %\newcommand{\matval}[1]{#1}

\newcommand{\sspace}{\quad}
\newcommand{\wspace}{\qquad}

\newcommand{\sand}{\sspace\text{and}\sspace}
\newcommand{\wand}{\wspace\text{and}\wspace}
\newcommand{\for}{\text{for }}

\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\unitvec}[2]{{\vecval{u}_{#1}^{(#2)}}}
\newcommand{\identitymat}[1]{\matval{\mathup{I}}_{#1,#1}}
\newcommand{\permutemat}{\matval{\Pi}}
\newcommand{\zerovec}[1]{\vecval{0}_{#1}}
\newcommand{\zeromat}[2]{\matval{0}_{#1,#2}}

\newcommand{\eqnannotate}[1]{\tag*{\color{AnnotationColor} #1}}
\newcommand{\eqnannotatefrom}[2][]{\eqnannotate{#1 from \Cref{#2}}}
\newcommand{\eqnannotatecf}[1]{\eqnannotate{\cf (\explicitref{#1})}}
\newcommand{\equalref}[1]{\,\stackrel{\text{\footnotesize(\explicitref{#1})}}{=}\,}

\newcommand{\fulfill}{\stackrel{!}{=}}
\newcommand{\inlineortho}{\bot}
\newcommand{\ortho}{\,\, \inlineortho \,\,}
\newcommand{\iszero}[1]{\underbrace{#1}_{=0}}

\newcommand{\vecsize}[1]{\in\R^{#1}}
\newcommand{\matsize}[2]{\in\R^{#1 \times #2}}

\newcommand{\Tsstep}[1]{\matval{\overline{#1}}}
\newcommand{\sstep}[1]{\matval{\overline{#1}}}
\newcommand{\Sstep}[1]{\matval{\ddot{#1}}}
\newcommand{\dual}[1]{\matval{\hat{#1}}}
\newcommand{\dualvec}[1]{\hat{#1}}
\newcommand{\append}[1]{\underline{#1}}

%\newcommand{\ATpower}[1]{{\left( \matval{A}\transpose \right)}^{#1}}
\newcommand{\ATpower}[1]{{( \matval{A}\transpose )}^{#1}}
\newcommand{\bracketT}[1]{{\left( #1 \right)}\transpose}

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\linearspan}[1]{\mathrm{span}\left( #1 \right)}
\newcommand{\conj}[1]{\overline{#1}}

\newcommand{\concatmat}[1]{\Concat{#1}}
\newcommand{\concatvec}[1]{\left[#1\right]}
\newcommand{\concatmatsep}{\, | \,}
%\newcommand{\lincomb}[1]{\left\langle #1 \right\rangle}
\newcommand{\lincomb}[1]{\linearspan{#1}}
%\newcommand{\vecprod}[2]{\left( #1, #2 \right)}
\newcommand{\vecprod}[2]{\left\langle #1, #2 \right\rangle}

%\newcommand{\sign}[1]{\mathrm{sign}\left( #1 \right)}
%\newcommand{\ssign}{\mathrm{sign}}
\newcommand{\diag}{\operatorname{diag}}
%\renewcommand\Re[1][]{\mathrm{Re}\,#1}
%\renewcommand\Im[1][]{\mathrm{Im}\,#1}

\newcommand{\vvector}[2]{\left[\begin{array}{c} #1 \\ #2 \end{array} \right]}
\newcommand{\vvvector}[3]{\left[\begin{array}{c} #1 \\ #2 \\ #3 \end{array} \right]}

\newcommand{\intervaloo}[2]{\left(#1,#2\right)}
\newcommand{\intervaloc}[2]{\left(#1,#2\right]}
\newcommand{\intervalco}[2]{\left[#1,#2\right)}
\newcommand{\intervalcc}[2]{\left[#1,#2\right]}

\newenvironment{mmatrix}{\begin{bmatrix}}{\end{bmatrix}}

\newcommand{\Oh}[1]{\mathrm{O}\left(#1\right)}

\newcommand{\e}[1]{\mathup{e}^{#1}}

\newcommand{\dd}{\mathop{}\!\mathrm{d}}
\newcommand{\Laplace}{\mathrm{\Delta}}

\newcommand\op[1]{{\hat{\mathrm{#1}}}}  % Operator

\newcommand\imaginary{\mathup{i}}

% use together with long limits in \sum, \prod, etc
% from mathmode, p. 63
  \def\clap#1{\hbox to 0pt{\hss#1\hss}}
  \def\mathclap{\mathpalette\mathclapinternal}
  \def\mathclapinternal#1#2{%
    \clap{$\mathsurround=0pt#1{#2}$}
  }


==> tex/macros/semantics.tex <==
%\newcommand\person[1]{#1} % für Personennamen
%\newcommand\software[1]{#1} % für Softwarenamen
%\newcommand\name[1]{\textsc{#1}} % für Personennamen
\newcommand\software[1]{\textsc{#1}} % für Softwarenamen

\newcommand\Index[1]{#1\index{#1}} % für Einträge, die im Text als auch im Index erscheinen sollen

\newcommand\cell[1]{\textcolor{gray}{#1}} % für Excel-Zellen
\newcommand\stress[1]{\emph{\Index{#1}}} % Hervorhebung von Schlüsselwörtern in Definitionen

\newcommand\change[1]{{\color{red}#1}}

==> tex/macros/tables.tex <==
%\newcolumntype{Q}{>{$}r<{$}}
%\newcolumntype{C}{>{$}c<{$}}
%\newcolumntype{J}{>{$}l<{$}}

%\newcolumntype{.}[1]{D{.}{,}{#1}}
%\newcolumntype{,}[1]{D{,}{,}{#1}}

%% Kommandos fuer Tabellen. Entnommen aus The LateX Companion, tabsatz.ps und diversen Dokus:

%%% -| Neue Spaltendefinitionen 'columntypes' |--
%
% Belegte Spaltentypen:
% l - links
% c - zentriert
% r - rechts
% p,m,b  - oben, mittig, unten
% X - tabularx Auto-Spalte

% um Tabellenspalten mit Flattersatz zu setzen, muss \\ vor
% (z.B.) \raggedright geschuetzt werden:
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}


% Spalten mit Flattersatz und definierte Breite:
% m{} -> mittig
% p{} -> oben
% b{} -> unten
%
% Linksbuendig:
\newcolumntype{v}[1]{>{\PreserveBackslash\RaggedRight\hspace{0pt}}p{#1}}
\newcolumntype{M}[1]{>{\PreserveBackslash\RaggedRight\hspace{0pt}}m{#1}}
% % Rechtsbuendig :
% \newcolumntype{R}[1]{>{\PreserveBackslash\RaggedLeft\hspace{0pt}}m{#1}}
% \newcolumntype{S}[1]{>{\PreserveBackslash\RaggedLeft\hspace{0pt}}p{#1}}
% % Zentriert :
% \newcolumntype{Z}[1]{>{\PreserveBackslash\Centering\hspace{0pt}}m{#1}}
% \newcolumntype{A}[1]{>{\PreserveBackslash\Centering\hspace{0pt}}p{#1}}

\newcolumntype{Y}{>{\PreserveBackslash\RaggedLeft\hspace{0pt}}X}
%%% Spalten fuer Mathematik
%
% serifenlose Matheschrift
%\newcolumntype{s}[1]{%
%  >{\DC@{.}{,}{#1}\mathsf\bgroup}l%
%  <{\egroup\DV@end}%
%}

% Tabellenspaltentyp fuer den Kopf: (Farbe + Ausrichtung)
\newcolumntype{H}[1]{>{\columncolor{tableheadcolor}}l}

% aequivalent aus typokurz (fett+grau+links)
% \newcolumntype{H}{>{\fontseries{b}\selectfont%
%     \columncolor[gray]{.8}[6pt][0pt]}l}
%%% --------------------------------------------


%%% ---|Listen in Tabellen |--------------------
\newcommand{\removeindentation}{%
  \leftmargini=\labelsep%
  \advance\leftmargini by \labelsep%
}
%
\makeatletter
\newcommand\tableitemize{
  \@minipagetrue%
  \removeindentation
}
\makeatother
%%% --------------------------------------------

%%% ---|Layout der Tabellen |-------------------

% Neue Umgebung fuer Tabellen:

\newenvironment{Tabelle}[2][c]{%
  \tablestylecommon
  \begin{longtable}[#1]{#2}
  }
  {\end{longtable}%
  \tablerestoresettings
}


% Groesse der Schrift in Tabellen
\newcommand{\tablefontsize}{ \footnotesize}
\newcommand{\tableheadfontsize}{\footnotesize}

% Layout der Tabelle: Ausrichtung, Schrift, Zeilenabstand
\newcommand\tablestylecommon{%
  \renewcommand{\arraystretch}{1.4} % Groessere Abstaende zwischen Zeilen
  \normalfont\normalsize            %
  \sffamily\tablefontsize           % Serifenlose und kleine Schrift
  \centering%                       % Tabelle zentrieren
}

\newcommand{\tablestyle}{
  \tablestylecommon
  %\tablealtcolored
}

% Ruecksetzten der Aenderungen
\newcommand\tablerestoresettings{%
  \renewcommand{\arraystretch}{1}% Abstaende wieder zuruecksetzen
  \normalsize\rmfamily % Schrift wieder zuruecksetzen
}

% Tabellenkopf: Serifenlos+fett+schraeg+Schriftfarbe
\newcommand\tablehead{%
  \tableheadfontsize%
  %\sffamily
  \bfseries%
  %\slshape
  %\color{white}
}

\newcommand\tablesubheadfont{%
  \tableheadfontsize%
  \sffamily\bfseries%
  \slshape
  %\color{white}
}


\newcommand\tableheadcolor{%
  %\rowcolor{tablesubheadcolor}
  %\rowcolor{tableblackheadcolor}
  \rowcolor{tableheadcolor}%
}

\newcommand\tablesubheadcolor{%
  \rowcolor{tablesubheadcolor}
  %\rowcolor{tableblackheadcolor}
}


\newcommand{\tableend}{\arrayrulecolor{black}\hline}

% Tabellenkopf (1=Spaltentyp, 2=Text)
% \newcommand{\tablehead}[2]{
%   \multicolumn{1}{#1@{}}{%
%     \raisebox{.1mm}{% Ausrichtung der Beschriftung
%       #2%
%     }\rule{0pt}{4mm}}% unsichtbare Linie, die die Kopfzeile hoeher macht
% }


\newcommand{\tablesubhead}[2]{%
  \multicolumn{#1}{>{\columncolor{tablesubheadcolor}}l}{\tablesubheadfont #2}%
}

% Tabellenbody (=Inhalt)
\newcommand\tablebody{%
\tablefontsize\sffamily\upshape%
}

\newcommand\tableheadshaded{%
  \rowcolor{tableheadcolor}%
}
\newcommand\tablealtcolored{%
  \rowcolors{1}{tablerowcolor}{white!100}%
}
%%% --------------------------------------------

\newlength{\mylen}
\newlength{\adjusthspace}

\newenvironment{tabularc}[2]
{%
  \setlength\mylen{#2/(#1)-\tabcolsep*2-\arrayrulewidth*(#1+1)/(#1)}%
  %\setlength{\adjusthspace}{((#2-1)/2)*\linewidth}
  %\par\noindent
  %\hspace*{-\the\adjusthspace}
  \begin{tabular}%{#2}%
    {*{#1}{v{\the\mylen}}}%
}
{\end{tabular}\par}

\newcommand{\mcellt}[2][l]{%
  \begin{tabular}[t]{@{}#1@{}}#2\end{tabular}}

==> tex/preamble.tex <==

\input{tex/preamble/encoding}
\input{tex/preamble/preamble-commands}
\input{tex/preamble/preloaded-packages}
\input{tex/preamble/maths}
\input{tex/preamble/symbols}
\input{tex/preamble/tables}
\input{tex/preamble/bibliography}
\input{tex/preamble/index}
\input{tex/preamble/referencing}
\input{tex/preamble/layout}

% ------------------------------------------------------------------------
% Document Informations:
% ------------------------------------------------------------------------

\title{\thesistitle}
\author{}
\date{\thesisdate}

\graphicspath{
      {fig/}
  }


\hyphenation{Re-si-du-al meth-od}

==> tex/preamble/bibliography.tex <==
%\usepackage[authordate-trad,backend=bibtex8,sorting=nyt,noibid,firstinits=true,uniquename=false]{biblatex-chicago}
%\usepackage{cite}
%\usepackage[natbibapa,nodoi]{apacite}
%\renewcommand{\BAvailFrom}{}
\usepackage{natbib}
\setlength{\bibsep}{0pt}
%\usepackage[style=ieee,backend=bibtex8]{biblatex}


%% ,backend=bibtex8,labeldate=true,datelabel=comp
%\usepackage[backend=biber,style=apa,maxcitenames=2,sortcites=true,doi=false,isbn=false,eventdate=comp,uniquename=false]{biblatex}
%\DeclareLanguageMapping{american}{american-apa}

% http://tex.stackexchange.com/questions/20605/biblatex-is-it-possible-to-combine-two-styles
%\renewcommand*{\nameyeardelim}{\addspace}

% Instead of the fix below we now use the xpatch package, see here:
% http://tex.stackexchange.com/questions/97206/how-to-tweak-3-5-authors-citation-with-the-biblatex-apa-style
%\usepackage{xpatch}
%\xpatchnameformat{labelname}
  %{\ifciteseen}{\ifnumcomp{\value{listtotal}}{>}{\value{maxnames}}}{}{}

%%% Fix: http://tex.stackexchange.com/questions/97031/how-to-modify-apa-biblatex-style-to-look-like-elsarticle-harv-style
%\makeatletter
%\DeclareNameFormat{labelname}{%
  %\ifthenelse{\value{uniquelist}>1}
    %{\numdef\cbx@min{\value{uniquelist}}}
    %{\numdef\cbx@min{\value{minnames}}}%
  %\ifboolexpr{test {\ifnumcomp{\value{listcount}}{=}{1}}
              %or test {\ifnumcomp{\value{listtotal}}{=}{2}}}
    %{\usebibmacro{labelname:doname}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}}
    %{\ifboolexpr{test {\ifnumcomp{\value{listtotal}}{>}{\value{maxnames}}}
                 %or test {\ifciteseen}}
     %{\ifnumcomp{\value{listcount}}{<}{\cbx@min + 1}% normal name
       %{\usebibmacro{labelname:doname}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}}%
       %{}%
      %\ifnumcomp{\value{listcount}}{=}{\cbx@min + 1}% first past ul is et al
       %%but enforce plurality of et al - only truncate here if there is at
       %%least one more element after the current potential truncation point
       %%so that "et al" covers at least two elements.
       %{\ifnumcomp{\value{listcount}}{<}{\value{listtotal}}
         %{\andothersdelim\bibstring{andothers}}
         %{\usebibmacro{labelname:doname}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}}}%
       %{}%
      %\ifnumcomp{\value{listcount}}{>}{\cbx@min + 1}% nothing thereafter
       %{\relax}%
       %{}}%
     %{\usebibmacro{labelname:doname}{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}}}}
%\makeatother

%\bibliography{bib/literature}
%
%%% Bug fix according to: http://gruppen.niuz.biz/biblatex-t791168.html?s=a2211626bab6f1f3835092194c5007ed&amp;
%\DeclareBibliographyDriver{booklet}{%
 %\usebibmacro{bibindex}%
 %\usebibmacro{begentry}%
 %\usebibmacro{author/editor}%
 %\setunit{\labelnamepunct}\newblock
 %\usebibmacro{title}%
 %\newunit\newblock
 %\printfield{howpublished}%
 %\newunit\newblock
 %\printfield{type}%
 %\newunit\newblock
 %\printfield{note}%
 %\newunit\newblock
 %% -------------------------------- alt:
 %% \usebibmacro{location+year}%
 %% -------------------------------- neu:
 %\usebibmacro{location+publisher}%
 %% --------------------------------
 %\newunit\newblock
 %\usebibmacro{doi+eprint+url}%
 %\newunit\newblock
 %\printfield{addendum}%
 %\newunit\newblock
 %\usebibmacro{related}%
%% \usebibmacro{apaageref}%
 %\usebibmacro{apa:finpunct}%
 %\usebibmacro{finentry}}

% -------------------------------------------------------------------------------------------------
%% declare author names as "last, first".
%% Either for the first author only or for all authors
%\DeclareNameFormat{author}{%
%    \ifthenelse{\value{listcount}=1}
%        {#1%                                            % first author
%            \ifblank{#3}{}{\addcomma\space #3}}
%        {#1%                                            % all the other authors (last, first)
%            \ifblank{#3}{}{\addcomma\space #3}}%
%%        {\ifblank{#3}{}{#3\space}%                      % all the other authors (first last)
%%            #1}%
%    \ifthenelse{\value{listcount}<\value{liststop}}
%        {,\space}
%            {}
%}
%
%%http://projekte.dante.de/DanteFAQ/BiblatexReihenfolgeAutoren
%\DeclareNameFormat{last-first}{%
%  \iffirstinits
%    {\usebibmacro{name:last-first}{#1}{#4}{#5}{#7}}
%    {\usebibmacro{name:last-first}{#1}{#3}{#5}{#7}}%
%  \usebibmacro{name:andothers}}
%\DeclareNameFormat{labelname}{%
%   \ifuseprefix
%     {\usebibmacro{name:last-first}{#1}{#4}{#5}{#8}}
%     {\usebibmacro{name:last-first}{#1}{#4}{#6}{#8}}%
%   \usebibmacro{name:andothers}}

%  \DefineBibliographyStrings{english}{%
%    typeeditor = {{}{}},
%    typeeditors = {{}{}},
%    in = {{}{}},
%    inseries = {{}{}},
%    byeditor = {{}{}}
%  }

%-------------------------------------------------------------------------------------------------

%%% http://www.golatex.de/biblatex-anpassen-die-x-te-frage-t4657.html
%\renewbibmacro*{journal+issuetitle}{%
%  \usebibmacro{journal}%
%  \setunit*{\addcomma\space}%
%  \iffieldundef{series}
%    {}
%    {\newunit
%     \printfield{series}%
%     \setunit{\addcomma\space}}%
%  \printfield{volume}%
%  \setunit*{\addcomma\space}%
%  \printfield{number}%
%  \setunit{\addcomma\space}%
%  \printfield{eid}%
%  \setunit{\addspace}%
%  \usebibmacro{issue+date}%
%  \setunit{\addcolon\space}%
%  \usebibmacro{issue}%
%  \newunit}
%
%\DeclareFieldFormat[article]{volume}{\bibstring{jourvol}~#1}
%\DeclareFieldFormat[article]{number}{\bibstring{number}~#1} 
%%\DeclareFieldFormat[article]{edition}{\bibstring{edition}~#1} 
%
%%% http://mrunix.de/forums/showthread.php?t=67386
%\DefineBibliographyStrings{english}{jourvol={Vol\adddot}} 
%\DefineBibliographyStrings{english}{number={No\adddot}} 
%\DefineBibliographyStrings{english}{edition={Ed\adddot}} 
%
%\AtBeginBibliography{%
  %% Setzt die Autoren-Vornamen auf Kapitälchen 
%%  \renewcommand*{\mkbibnamefirst}{\textsc}
%%  \renewcommand*{\mkbibnamelast}{\textsc}
%%  \renewcommand*{\mkbibnameprefix}{\textsc}
%%  \renewcommand*{\mkbibnameaffix}{\textsc}
  %
  %%%Doppelpunkt nach Namen, kein Punkt
  %%\renewcommand*{\labelnamepunct}{\addcolon\space} 
  %
%%  \DeclareFieldFormat{name}{\textsc{#1\isdot}}
%%  \DeclareFieldFormat{title}{\mkbibemph{#1\isdot}}
%
%%  \DeclareFieldFormat{title}{#1}
  %\DeclareFieldFormat{journaltitle}{#1}    % remove italics from journal title
  %\DeclareFieldFormat{booktitle}{#1}    % remove italics from journal title
  %
  %%%\DeclareFieldFormat[article]{title}{#1}
  %%%\DeclareFieldFormat[article]{title}{\mkbibquote{#1}}
%%  \renewcommand*{\mkbibquote}[1]{\mkbibemph{#1\isdot}}
 %
  %% http://tex.stackexchange.com/ ...
  %% questions/16716/spell-out-volume-and-edition-in-words-biblatex-in-german
  %%\renewcommand*{\mkbibordedition}[1]{\Ordinalstringnum{#1}[f]}
%%  \renewcommand*{\mkbibordedition}[1]{\ordinalnum{#1}}
%}
%
%\setlength{\bibhang}{0.5cm}
%%\AtEveryBibitem{\bibhang}

==> tex/preamble/coding.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% verbatim packages
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/upquote/upquote.sty
\usepackage{upquote} % Setzt "richtige" Quotes in verbatim-Umgebung
 
%%% Doc: No Documentation;
  \usepackage{verbatim} %Reimplemntation of the original verbatim
 
%%% Doc: http://www.cs.brown.edu/system/software/latex/doc/fancyvrb.pdf
% \usepackage{fancyvrb} % Superior Verbatim Class

\IfPackageLoaded{fancyvrb}{
  \DefineShortVerb{\|} % Nur mit fancyvrb zusammen laden!
}
 
%% Listings Paket ------------------------------------------------------
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/listings/listings-1.3.pdf
% für source code listings; verwenden mit \lstinline|...|, \begin{lstlisting}...\end{lstlisting} oder \lstinputlisting{file}
\usepackage{listings}
  \lstset{%
    basicstyle=\scriptsize\ttfamily,
    tabsize=3,
    showtabs=false,
    showspaces=false,
    showstringspaces=false,
    tab=\rightarrowfill,
    keywordstyle=\color{ListingsKeywordColor},
    identifierstyle=\color{ListingsIdentifierColor},
    commentstyle=\color{ListingsCommentColor},
    stringstyle=\color{ListingsStringColor},
    emphstyle=\color{ListingsEmphColor}\bfseries\underbar,
    frame=none,
    rulesepcolor=\color{ListingsRuleSepColor},
    numbers=left, 
    numberstyle=\tiny, 
    numbersep=5pt,
    captionpos=top,
    frame=tb,
    firstnumber=1,
    stepnumber=5,
    numberfirstline=false,
    breaklines=true,
    breakatwhitespace=true,
    prebreak=\mbox{\,$\color{ListingsBreakSymbolColor}\mathbf{\hookleftarrow}$},
    mathescape=true,
    morekeywords={},
}
%  \lstset{%
%         basicstyle=\small\ttfamily, % Standardschrift
%         numbers=left,               % Ort der Zeilennummern
%         numberstyle=\tiny,          % Stil der Zeilennummern
%         stepnumber=2,               % Abstand zwischen den Zeilennummern
%         numbersep=5pt,              % Abstand der Nummern zum Text
%         tabsize=2,                  % Groesse von Tabs
%         extendedchars=true,         %
%         breaklines=true,            % Zeilen werden Umgebrochen
% %        keywordstyle=[1]\textbf,    % Stil der Keywords
% %        keywordstyle=[2]\textbf,    %
% %        keywordstyle=[3]\textbf,    %
% %        keywordstyle=[4]\textbf,    %
%         stringstyle=\color{stringcolor}, % Farbe der String
%         showspaces=false,           % Leerzeichen anzeigen ?
%         showtabs=false,             % Tabs anzeigen ?
%         showstringspaces=false      % Leerzeichen in Strings anzeigen ?
%  }
  \lstloadlanguages{% Check Dokumentation for further languages ...
           [Sharp]C
%         [Visual]Basic
%         %Pascal
%         %C
%         %C++
%         %XML
%         %HTML
  }
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/examplep/eurotex_2005_examplep.pdf
% LaTeX Code und Ergebnis nebeneinander darstellen
%\usepackage{examplep}
%\usepackage[boxed,ruled]{algorithm2e}
%\usepackage[chapter]{algorithm}

%\usepackage{algorithmic}        % für Pseudo-Code-Algorithmen
%  \renewcommand{\algorithmicrequire}{\reallynopagebreak\textbf{Input:}}
%  \renewcommand{\algorithmicensure}{\reallynopagebreak\textbf{Output:}}
  
\usepackage[ruled]{algorithm2e}          % für Algorithmus-Einbettungs-Umgebung

  \makeatletter
\newenvironment{inlinealgorithm}[1]{%
  \medskip%
  \noindent\parbox{\linewidth}{\def\@fs@cfont{\bfseries}%
  \let\@fs@capt\relax%
  \par\noindent%
  \rule{\linewidth}{.8pt}%
  \vspace{-10pt}%
  \noindent\captionof{algorithm}{#1}%
  \vspace{-0.7\baselineskip}%
  \noindent\rule{\linewidth}{.4pt}%
  \vspace{0.2\baselineskip}}%
%  \vspace{-1.3\baselineskip}\reallynopagebreak%
%% My hack, as algorithmic uses the overall number of lines in the whole document for labels, instead of using the description from within a single algorithm
  \renewcommand*\theALC@unique{\theALC@line}%
  \reallynopagebreak%
}{%
  \vspace{-.75\baselineskip}%
  \rule{\linewidth}{.4pt}%
  \medskip%
}

\newenvironment{inlinelisting}[1]{%
  \def\@fs@cfont{\bfseries}%
  \let\@fs@capt\relax%
  \par\noindent%
  %\medskip%
  \rule{\linewidth}{.8pt}%
  \vspace{-10pt}%
%  \noindent\captionof{algorithm}{#1}%
  \vspace{-0.35\baselineskip}%
}{}
\makeatother

==> tex/preamble/colors.tex <==
    \definecolor{BottomBoxColor}{rgb}{0,0,0}
    \definecolor{HiddenContentColor}{rgb}{0.5,0.5,0.5}
    \definecolor{MarginNoteColor}{rgb}{0,0,0.8}
    \definecolor{ListingsKeywordColor}{rgb}{0,0,0.4}
    \definecolor{ListingsIdentifierColor}{rgb}{0,0.5,0}
    \definecolor{ListingsCommentColor}{rgb}{0.4,0.4,0.4}
    \definecolor{ListingsStringColor}{rgb}{0.6000,0.3333,0.7333}%{0.8,0,0}
    \definecolor{ListingsRuleSepColor}{rgb}{0,0,0}
    \definecolor{ListingsEmphColor}{rgb}{0,0.6667,0.6667}
    \definecolor{ListingsBreakSymbolColor}{rgb}{0.780,0.082,0.522}
    \definecolor{SectionColor}{rgb}{0,0,0}
    \definecolor{MathsCancelColor}{rgb}{0.5,0.5,0.5}
    \definecolor{AnnotationColor}{rgb}{0,0,0}

\IfDefined{thesistypedebug}{%
    \definecolor{LinkColor}{rgb}{0,0,0.5}
    \definecolor{UnitColor}{rgb}{0,0.6,1}
    \definecolor{MathsVectorColor}{rgb}{0,0.5,0}
    \definecolor{MathsMatrixColor}{rgb}{0.5,0,0}
}
\IfDefined{thesistypeprint}{%
    \definecolor{LinkColor}{rgb}{0,0,0}
    \definecolor{UnitColor}{rgb}{0,0,0}    
    \definecolor{MathsVectorColor}{rgb}{0,0,0}
    \definecolor{MathsMatrixColor}{rgb}{0,0,0}
}
\IfDefined{thesistypescreen}{%
    \definecolor{LinkColor}{rgb}{0,0,0.5}
    \definecolor{UnitColor}{rgb}{0,0,0}    
    \definecolor{MathsVectorColor}{rgb}{0,0,0}
    \definecolor{MathsMatrixColor}{rgb}{0,0,0}
}

==> tex/preamble/encoding.tex <==
% Encoding der Dateien (sonst funktionieren Umlaute nicht)
% Fuer Linux -> utf8
% Fuer Windows, alte Linux Distributionen -> latin1
 
% Empfohlen latin1, da einige Pakete mit utf8 Zeichen nicht
% funktionieren, z.B: listings, soul. 
\usepackage[latin1]{inputenc}
%\usepackage[ansinew]{inputenc}
%\usepackage[utf8]{inputenc}
%\usepackage{ucs}
%\usepackage[utf8x]{inputenc}

==> tex/preamble/figures.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% figures and placement
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
 
\makeatletter
    \renewcommand{\fps@figure}{htbp}         % default {tbp}
\makeatother 

%% Bilder und Graphiken ==================================================
 
%%% Doc: only dtx Package
\usepackage{float}             % Stellt die Option [H] fuer Floats zur Verfgung
  
%%% Doc: No Documentation
\usepackage{flafter}          % Floats immer erst nach der Referenz setzen
 
% Defines a \FloatBarrier command, beyond which floats may not
% pass; useful, for example, to ensure all floats for a section
% appear before the next \section command.
\usepackage[
  section    % "\section" command will be redefined with "\FloatBarrier"
]{placeins}
  % Bug fix: FloatBarrier for subsection
    \makeatletter
  \AtBeginDocument{%
     \expandafter\renewcommand\expandafter\subsection\expandafter
       {\expandafter\@fb@secFB\subsection}%
     %\newcommand\@fb@secFB{\FloatBarrier
     %\gdef\@fb@afterHHook{\@fb@topbarrier \gdef\@fb@afterHHook{}}}
     \g@addto@macro\@afterheading{\@fb@afterHHook}
     \gdef\@fb@afterHHook{}
  }
    \makeatother



%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/subfig/subfig.pdf
% Incompatible: loads package capt-of. Loading of 'capt-of' afterwards will fail therefor
%\usepackage{subfig} % Layout wird weiter unten festgelegt !
 
%%% Bilder von Text Umfliessen lassen : (empfehle wrapfig)
%
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/wrapfig/wrapfig.sty
\usepackage{wrapfig}          % defines wrapfigure and wrapfloat
%\setlength{\wrapoverhang}{\marginparwidth} % aeerlapp des Bildes ...
%\addtolength{\wrapoverhang}{\marginparsep} % ... in den margin
\setlength{\intextsep}{0.5\baselineskip} % Platz ober- und unterhalb des Bildes
% \intextsep ignoiert bei draft ???
%\setlength{\columnsep}{1em} % Abstand zum Text
 
%%% Doc: Documentation inside dtx Package
%\usepackage{floatflt}       % LaTeX2e Paket von 1996
                             % [rflt] - Standard float auf der rechten Seite
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex209/contrib/picins/picins.doc
%\usepackage{picins}          % LaTeX 2.09 Paket von 1992. aber Layout kombatibel
 
 
% Make float placement easier
\renewcommand{\floatpagefraction}{.75} % vorher: .5
\renewcommand{\textfraction}{.1}       % vorher: .2
\renewcommand{\topfraction}{.8}        % vorher: .7
\renewcommand{\bottomfraction}{.5}     % vorher: .3
\setcounter{topnumber}{3}              % vorher: 2
\setcounter{bottomnumber}{2}           % vorher: 1
\setcounter{totalnumber}{5}            % vorher: 3
 
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/psfrag/pfgguide.pdf
  \usepackage{psfrag}  % Ersetzen von Zeichen in eps Bildern
 
 
%%% Doc: http://www.ctan.org/tex-archive/macros/latex/contrib/sidecap/sidecap.pdf
\usepackage[%
%  outercaption,%  (default) caption is placed always on the outside side
%  innercaption,% caption placed on the inner side
%  leftcaption,%  caption placed on the left side
  rightcaption,% caption placed on the right side
%  wide,%      caption of float my extend into the margin if necessary
%  margincaption,% caption set into margin
  ragged,% caption is set ragged
]{sidecap}
 
\renewcommand\sidecaptionsep{2em}
%\renewcommand\sidecaptionrelwidth{20}
\sidecaptionvpos{table}{c}
\sidecaptionvpos{figure}{c}

\usepackage{framed}

% ------------------------------------------------------------------------
% PStricks stuff
% ------------------------------------------------------------------------

%    \usepackage{pst-plot}

\usepackage{tikz}
  \usetikzlibrary{matrix,arrows,decorations.pathmorphing}
  
%% \usepackage{rotating}
  
%% Diagramme mit LaTeX ===================================================
%
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/pict2e/pict2e.pdf
% Neuimplementation der Picture Umgebung.
%
% The new package extends the existing LaTeX picture environment, using
% the familiar technique (cf. the graphics and color packages) of driver
% files.  The package documentation (pict2e.dtx) has a fair number of
% examples of use, showing where things are improved by comparison with
% the LaTeX picture environment.
% \usepackage{pict2e}
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/curve2e/curve2e.pdf
% Extensions for package pict2e.
%\usepackage{curve2e}
%

\usepackage{pgfplots}
\usepackage{pgfplotstable}
  \usepgfplotslibrary{groupplots}
  \usetikzlibrary{pgfplots.groupplots}

  \pgfplotscreateplotcyclelist{blue}{%
    violet,
    teal,
    cyan,
    Blue,
    pink,
    magenta,
    RawSienna
  }
  \pgfplotsset{%
    compat=newest,
    legend style={font=\footnotesize},
    label style={font=\footnotesize},
    tick label style={font=\footnotesize},
    every mark/.append style={scale=0.7},
    no markers,
    width=0.95\linewidth,
    height=7cm,
    legend cell align=left,
    every axis/.append style={line width=0.5pt},
    cycle list name=blue,
    xlabel=Iteration index $n$,
    grid=major,
    every axis grid/.append style={dotted,black!40},
    enlarge x limits=0.05,
    %axis x line=bottom,
    %axis y line=left
  }  

  %% Hack: Disable tikzpicture in draft mode
  \IfDraft{%
    % Requires: verbatim for \comment
    \newcommand{\mydrafttikzpicture}{\rule{0.9\textwidth}{8cm}\comment}
    \let\tikzpicture=\mydrafttikzpicture
    \let\endtikzpicture=\endcomment
  }

==> tex/preamble/fonts.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Fonts Fonts Fonts
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
 
\usepackage[T1]{fontenc} % T1 Schrift Encoding
\usepackage{textcomp}   % Zusatzliche Symbole (Text Companion font extension)

% Alle Schriften die hier angegeben sind sehen im PDF richtig aus.
% Die LaTeX Standardschrift ist die Latin Modern (lmodern Paket).
% If Latin Modern is not available for your distribution you must install the
% package cm-super instead. Otherwise your fonts will look horrible in the PDF
 
% DO NOT LOAD ae Package for the font !

%%% Textverzierungen/Auszeichnungen ======================================
%
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/misc/ulem.sty
%\usepackage[normalem]{ulem}      % Zum Unterstreichen
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/soul/soul.pdf
%\usepackage{soul}                % Unterstreichen, Sperren
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/misc/url.sty
\usepackage{url} % Setzen von URLs. In Verbindung mit hyperref sind diese auch aktive Links.

%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/lettrine/doc/lettrine.pdf
% Dropping capitals
% \usepackage{lettrine}
 
%% ==== Zusammengesetzte Schriften  (Sans + Serif) =======================
 
%% - Stefans Style
  % load sans-serif font
%\usepackage{lmodern}
%\usepackage[scaled]{helvet}        %% --- Helvetica
%\usepackage{cmbright}                  %% --- CM-Bright (eigntlich eine Familie)
%\usepackage{tpslifonts}                %% --- tpslifonts % Font for Slides
%\usepackage{avantgar}                  %% --- Avantgarde
  % font in math mode
%\usepackage{mathptmx}
  % default font: charter
%\usepackage{charter}\linespread{1.05} 
%\usepackage{times}
  % switch sans-serif to lmodern
%\renewcommand{\sfdefault}{lmss}

% Fix: mathptmx has no support for bold math
%http://www.foonews.info/de-comp-text-tex/2435035-re-fette-caligraphische-buchstaben-mit-bm-mathcal-n.html
  \renewcommand\boldmath{\mathversion{bold}}

  \SetSymbolFont{operators}   {bold}  {OT1}{lmr} {bx}{n}
  \SetSymbolFont{letters}     {bold}  {OML}{lmm} {b}{it}
  \SetSymbolFont{symbols}     {bold}  {OMS}{lmsy}{b}{n}
  \SetSymbolFont{largesymbols}{bold}  {OMX}{lmex}{m}{n}
  %\SetMathAlphabet{\mathbf}{bold}  {OT1}{lmr}{bx}{n}
  %\SetMathAlphabet{\mathsf}{bold}  {OT1}{lmss}{bx}{n}
  %\SetMathAlphabet{\mathit}{bold}  {OT1}{lmr}{bx}{it}
  %\SetMathAlphabet{\mathtt}{bold}  {OT1}{lmtt}{m}{n}


%% - Latin Modern
%\usepackage{lmodern}

%% -------------------
%
%% - Times, Helvetica, Courier (Word Standard...)
%\usepackage{mathptmx}
%\usepackage[scaled=.90]{helvet}
%\usepackage{courier}
%% -------------------
%%
%% - Palantino , Helvetica, Courier
%\usepackage{mathpazo}
%\usepackage[scaled=.95]{helvet}
%\usepackage{courier}
%% -------------------
%
%% - Bera Schriften
%\usepackage{bera}
%% -------------------
%
%% - Charter, Bera Sans
%\usepackage{charter}\linespread{1.05}
%\renewcommand{\sfdefault}{fvs}
 
%% ===== Serifen =========================================================
 
%\usepackage{mathpazo}                 %% --- Palantino
\usepackage{charter}\linespread{1.05} %% --- Charter
%\usepackage{bookman}                  %% --- Bookman (laedt Avant Garde !!)
%\usepackage{newcent}                  %% --- New Century Schoolbook (laedt Avant Garde !!)
 
%\usepackage[%                         %% --- Fourier
%   upright,     % Math fonts are upright
%   expert,      % Only for EXPERT Fonts!
%   oldstyle,    % Only for EXPERT Fonts!
%   fulloldstyle % Only for EXPERT Fonts!
%]{fourier} %
 
 
 
%% ===== Sans Serif ======================================================
 
%\usepackage[scaled=.95]{helvet}        %% --- Helvetica
%\usepackage{cmbright}                  %% --- CM-Bright (eigntlich eine Familie)
%\usepackage{tpslifonts}                %% --- tpslifonts % Font for Slides
%\usepackage{avantgar}                  %% --- Avantgarde
 
%%%% =========== Italics ================
 
%\usepackage{chancery}                  %% --- Zapf Chancery
 
%%%% =========== Typewriter =============
 
%\usepackage{courier}                   %% --- Courier
%\renewcommand{\ttdefault}{cmtl}        %% --- CmBright Typewriter Font
%\usepackage[%                          %% --- Luxi Mono (Typewriter)
%   scaled=0.9
%]{luximono}
 
 
 
%%%% =========== Mathe ================
 
%% Recommanded to use with fonts: Aldus, Garamond, Melior, Sabon
%\usepackage[                           %% --- EulerVM (MATH)
%   small,       %for smaller Fonts
%  euler-digits % digits in euler fonts style
%]{eulervm}
 
% \usepackage[
% %   utopia,
% %   garamond,
%    charter
% ]{mathdesign}
 
%%%% (((( !!! kommerzielle Schriften !!! )))))))))))))))))))))))))))))))))))))))))))))))))))
 
%% ===== Serifen (kommerzielle Schriften ) ================================
 
%% --- Adobe Aldus
%\renewcommand{\rmdefault}{pasx}
%\renewcommand{\rmdefault}{pasj} %%oldstyle digits
% math recommended: \usepackage[small]{eulervm}
 
%% --- Adobe Garamond
%\usepackage[%
%   osf,        % oldstyle digits
%   scaled=1.05 %appropriate in many cases
%]{xagaramon}
% math recommended: \usepackage{eulervm}
 
%% --- Adobe Stempel Garamond
%\renewcommand{\rmdefault}{pegx}
%\renewcommand{\rmdefault}{pegj} %%oldstyle digits
 
%% --- Adobe Melior
%\renewcommand{\rmdefault}{pml}
% math recommended: %\usepackage{eulervm}
 
%% --- Adobe Minion
%\renewcommand{\rmdefault}{pmnx}
%\renewcommand{\rmdefault}{pmnj} %oldstyle digits
% math recommended: \usepackage[small]{eulervm} or \usepackage{mathpmnt} % commercial
 
%% --- Adobe Sabon
%\renewcommand{\rmdefault}{psbx}
%\renewcommand{\rmdefault}{psbj} %oldstyle digits
% math recommended: \usepackage{eulervm}
 
%% --- Adobe Times
% math recommended: \usepackage{mathptmx} % load first !
%\renewcommand{\rmdefault}{ptmx}
%\renewcommand{\rmdefault}{ptmj} %oldstyle digits
 
%% --- Linotype ITC Charter
%\renewcommand{\rmdefault}{lch}
 
%% --- Linotype Meridien
%\renewcommand{\rmdefault}{lmd}
 
%%% ===== Sans Serif (kommerzielle Schriften) ============================
 
%% --- Adobe Frutiger
%\usepackage[
%   scaled=0.90
%]{frutiger}
 
%% --- Adobe Futura (=Linotype FuturaLT) : Sans Serif
%\usepackage[
%   scaled=0.94  % appropriate in many cases
%]{futura}
 
%% --- Adobe Gill Sans : Sans Serif
%\usepackage{gillsans}
 
%% -- Adobe Myriad  : Sans Serif
%\renewcommand{\sfdefault}{pmy}
%\renewcommand{\sfdefault}{pmyc} %% condensed Font
 
%% --- Syntax : sans serif font
%\usepackage[
%   scaled
%]{asyntax}
 
%% --- Adobe Optima : Semi Sans Serif
%\usepackage[
%   medium %darker medium weight fonts
%]{optima}
 
%% --- Linotype ITC Officina Sans
%\renewcommand{\sfdefault}{lo9}

==> tex/preamble/footnotes.tex <==
%%% Fussnoten/Endnoten ===================================================
%
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/footmisc/footmisc.pdf
%
\usepackage[
   bottom,      % Footnotes appear always on bottom. This is necessary
                % especially when floats are used
   stable,      % Make footnotes stable in section titles
   perpage,     % Reset on each page
   %para,       % Place footnotes side by side of in one paragraph.
   %side,       % Place footnotes in the margin
   ragged,      % Use RaggedRight
   %norule,     % suppress rule above footnotes
   multiple,    % rearrange multiple footnotes intelligent in the text.
   %symbol,     % use symbols instead of numbers
]{footmisc}
 
%% Einruecken der Fussnote einstellen
%\setlength\footnotemargin{10pt}
 
%--- footnote counter documentweit durchlaufend ------------------------------
%\usepackage{chngcntr}
%\counterwithout{footnote}{chapter}
%-----------------------------------------------------------------------------
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/misc/endnotes.sty
%\usepackage{endnotes}
% From the Documentation:
% To turn all the footnotes in your documents into endnotes, say
%
%     \let\footnote=\endnote
%
%  in your preamble, and then add something like
%
%     \newpage
%     \begingroup
%     \parindent 0pt
%     \parskip 2ex
%     \def\enotesize{\normalsize}
%     \theendnotes
%     \endgroup
%
% as the last thing in your document.  (But \theendnotes all
% by itself will work.)

==> tex/preamble/index.tex <==
\usepackage{makeidx}    % Index
\IfDraft{
  \IfDefined{makeindex}{\usepackage{showidx}}    % Indexierte Begriffe am Rand (Korrekturlesen)
}

%%% Index & Co. ===========================================================
%% gibts dafuer noch eine sauberere Loesung ?
%%%%%%%%% Index zweispaltig %%%%%%%
%% \makeatletter
%% \renewenvironment{theindex}{%
%% \setlength{\columnsep}{2em}
%% \begin{multicols}{2}[\section*{\indexname}]
%% \parindent\z@
%% \parskip\z@ \@plus .3\p@\relax
%% \let\item\@idxitem}%
%% {\end{multicols}\clearpage}
%% \makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/nomencl/nomencl.pdf
%\usepackage[%
%  %german,
%  english
%]{nomencl}[2005/09/22]

% Symbolverzeichnis
%\usepackage[english,notintoc]{nomentbl}
%    \def\nompreamble{Hier evtl. Text \par\bigskip}


==> tex/preamble/layout.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% layout packages
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

%%% Diverse Pakete und Einstellungen =====================================
 
%%% Doc: Documentation inside dtx file
% Mehrere Text-Spalten
\usepackage{multicol}

\usepackage{lscape}
\usepackage{rotating}
 
%\nonfrenchspacing     % liefert extra Platz hinter Satzenden.
                                % Fuer deutschen Text standardmaessig ausgeschaltet!
 
\usepackage{ellipsis}  % >>Intelligente<< \dots

%% bei Zweiseitigem Druck besser auskommentieren
\clubpenalty = 10000        % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000       % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

%% Zeilenabstand =========================================================
%
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/setspace/setspace.sty
\usepackage{setspace}
%\doublespace          % 2-facher Abstand
%\onehalfspace        % 1,5-facher Abstand
% hereafter load 'typearea' again

%% Seitenlayout ==========================================================
%
%% Layout laden um im Dokument den Befehl \layout nutzen zu koennen
%%%% Doc: no documentation
%%\usepackage[verbose]{layout}
%%
 
% Layout mit 'geometry'
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/geometry/manual.pdf
\usepackage{geometry}
 
\IfPackageLoaded{geometry}{%
\geometry{%
%%% Paper Groesse
   letterpaper, % Andere a0paper, a1paper, a2paper, a3paper, , a5paper, a6paper,
            % b0paper, b1paper, b2paper, b3paper, b4paper, b5paper, b6paper
            % letterpaper, executivepaper, legalpaper
   %screen,  % a special paper size with (W,H) = (225mm,180mm)
   %paperwidth=,
   %paperheight=,
   %papersize=, %{ width , height }
   %landscape,  % Querformat
   portrait,    % Hochformat
%%% Koerper Groesse
   %hscale=,      % ratio of width of total body to \paperwidth
                  % hscale=0.8 is equivalent to width=0.8\paperwidth. (0.7 by default)
   %vscale=,      % ratio of height of total body to \paperheight
                  % vscale=0.9 is equivalent to height=0.9\paperheight.
   %scale=,       % ratio of total body to the paper. scale={ h-scale , v-scale }
   %totalwidth=,    % width of total body % (Generally, width >= textwidth)
   %totalheight=,   % height of total body, excluding header and footer by default
   %total=,        % total={ width , height }
   %textwidth=,    % modifies \textwidth, the width of body
   %textheight=,   % modifies \textheight, the height of body
   %body=,        % { width , height } sets both \textwidth and \textheight of the body of page.
 %  lines=50,       % enables users to specify \textheight by the number of lines.
   %includefoot,  % includes the foot of the page, \footskip, into body.
   %includehead,  % includes the head of the page, \headheight and \headsep, into total body.
   %includeheadfoot, % sets both includehead and includefoot to true
   %includemp,    % includes the margin notes, \marginparwidth and \marginparsep, into body
   %includeall,   % sets both includeheadfoot and includemp to true.
   %ignorehead,   % disregards the head of the page, headheight and headsep in determining vertical layout
   %ignorefoot,   % disregards the foot of page, footskip, in determining vertical layout
   %ignoreheadfoot, % sets both ignorehead and ignorefoot to true.
   %ignoremp,     % disregards the marginal notes in determining the horizontal margins
   ignoreall,     % sets both ignoreheadfoot and ignoremp to true
   heightrounded, % This option rounds \textheight to n-times (n: an integer) of \baselineskip
   %hdivide=,     % { left margin , width , right margin }
                  % Note that you should not specify all of the three parameters
   %vdivide=,     % { top margin , height , bottom margin }
   %divide=,      % ={A,B,C} %  is interpreted as hdivide={A,B,C} and vdivide={A,B,C}.
 %Margin
   lmargin=1in,        % left margin (for oneside) or inner margin (for twoside) of total body
                  % alias: lmargin, inner
   rmargin=1in,       % right or outer margin of total body
                  % alias: rmargin outer
   tmargin=1in,         % top margin of the page.
                  % Alias : tmargin
   bmargin=1in,      % bottom margin of the page
                  % Alias : bmargin
   %hmargin=,     % left and right margin. hmargin={ left margin , right margin }
   %vmargin=,     % top and bottom margin. vmargin={ top margin , bottom margin }
   %margin=,      % margin={A,B} is equivalent to hmargin={A,B} and vmargin={A,B}
   %hmarginratio, % horizontal margin ratio of left (inner) to right (outer).
   %vmarginratio, % vertical margin ratio of top to bottom.
   %marginratio,  % marginratio={ horizontal ratio , vertical ratio }
   %hcentering,   % sets auto-centering horizontally and is equivalent to hmarginratio=1:1
   %vcentering,   % sets auto-centering vertically and is equivalent to vmarginratio=1:1
   %centering,    % sets auto-centering and is equivalent to marginratio=1:1
  % twoside,       % switches on twoside mode with left and right margins swapped on verso pages.
   %asymmetric,   % implements a twosided layout in which margins are not swapped on alternate pages
                  % and in which the marginal notes stay always on the same side.
 %  bindingoffset=5mm,  % removes a specified space for binding
%%% Dimensionen
   %headheight=,  % Alias:  head
   %headsep=,     % separation between header and text
   %footskip=,    % distance separation between baseline of last line of text and baseline of footer
                  % Alias: foot
   %nohead,       % eliminates spaces for the head of the page
                  % equivalent to both \headheight=0pt and \headsep=0pt.
   %nofoot,       % eliminates spaces for the foot of the page
                  % equivalent to \footskip=0pt.
   %noheadfoot,   % equivalent to nohead and nofoot.
   %footnotesep=, % changes the dimension \skip\footins,.
                  % separation between the bottom of text body and the top of footnote text
  % marginparwidth=0pt, % width of the marginal notes
                  % Alias: marginpar
   %marginparsep=,% separation between body and marginal notes.
   %nomarginpar,  % shrinks spaces for marginal notes to 0pt
   %columnsep=,   % the separation between two columns in twocolumn mode.
   %hoffset=,
   %voffset=,
   %offset=,      % horizontal and vertical offset.
                  % offset={ hoffset , voffset }
   %twocolumn,    % twocolumn=false denotes onecolumn
   %twoside,
   %textwidth=380pt,   % sets \textwidth directly
   %textheight=,  % sets \textheight directly
   %reversemp,    % makes the marginal notes appear in the left (inner) margin 
                  % Alias: reversemarginpar
}
} % Endif
 
% - Anzeigen des Layouts -
\IfPackageLoaded{geometry}{%
   %\geometry{showframe}
}
 
% Layout mit 'typearea'
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/koma-script/scrguide.pdf
\usepackage{typearea} 
 
\IfPackageLoaded{typearea}{% Wenn typearea geladen ist
   \IfPackageNotLoaded{geometry}{% aber nicht geometry
      \typearea[current]{last}
   }
}
 
% BCOR
%    current  % Satzspiegelberechnung mit dem aktuell gültigen BCOR-Wert erneut
%             % durchführen.
% DIV
%    calc     % Satzspiegelberechnung einschließlich Ermittlung eines guten
%             % DIV-Wertes erneut durchführen.
%    classic  % Satzspiegelberechnung nach dem
%             % mittelalterlichen Buchseitenkanon
%             % (Kreisberechnung) erneut durchführen.
%    current  % Satzspiegelberechnung mit dem aktuell gültigen DIV-Wert erneut
%             % durchführen.
%    default  % Satzspiegelberechnung mit dem Standardwert für das aktuelle
%             % Seitenformat und die aktuelle Schriftgröße erneut durchführen.
%             % Falls kein Standardwert existiert calc anwenden.
%    last     % Satzspiegelberechnung mit demselben DIV -Argument, das beim
%             % letzten Aufruf angegeben wurde, erneut durchführen
 
 
%\usepackage[colorgrid,texcoord,gridunit=mm]{showframe}
 
\raggedbottom     % Variable Seitenhoehen zulassen

%%% Aussehen der URLS======================================================
 
%fuer URL (nur wenn url geladen ist)
\IfDefined{urlstyle}{
  \urlstyle{rm} %sf
}

%%% Kopf und Fusszeilen====================================================
%%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/koma-script/scrguide.pdf
\usepackage[%
   automark,         % automatische Aktualisierung der Kolumnentitel
   nouppercase,      % Grossbuchstaben verhindern
   %markuppercase    % Grossbuchstaben erzwingen
   %markusedcase     % vordefinierten Stil beibehalten
   %komastyle,       % Stil von Koma Script
   %standardstyle,   % Stil der Standardklassen
]{scrpage2}
% 
%\IfElseChapterDefined{%
%   \pagestyle{scrheadings} % Seite mit Headern
%}{
%   \pagestyle{scrplain} % Seiten ohne Header
%}
%%\pagestyle{empty} % Seiten ohne Header
%%
%% loescht voreingestellte Stile
%\clearscrheadings
%\clearscrplain
%%
%% Was steht wo...
%\IfElseChapterDefined{
%   % Oben aussen: Kapitel und Section
%   % Unten aussen: Seitenzahl
%   % \ohead{\headmark} % Oben außen: Setzt Kapitel und Section automatisch
%   % \ofoot[\pagemark]{\pagemark}
%   % oder...
%   % Oben aussen: Seitenzahlen
%   % Oben innen: Kapitel und Section
%   \ohead{\pagemark}
%   \ihead{\headmark}
%}{
%   \cfoot[\pagemark]{\pagemark} % Mitte unten: Seitenzahlen bei plain
%}
\chead{}
\lehead{\emph{\papertrack}}
\rohead{\emph{\papershorttitle}}

\cfoot{}
\lefoot{\emph{\textbf{\pagemark}\quad Thirty ninth International Conference on Information Systems, San Francisco 2018}}
\rofoot{\emph{Thirty ninth International Conference on Information Systems, San Francisco 2018\quad\textbf{\pagemark}}}

%% Vollstaendige Liste der moeglichen Positionierungen
%% \lehead[scrplain-links-gerade]{scrheadings-links-gerade}
%% \cehead[scrplain-mittig-gerade]{scrheadings-mittig-gerade}
%% \rehead[scrplain-rechts-gerade]{scrheadings-rechts-gerade}
%% \lefoot[scrplain-links-gerade]{scrheadings-links-gerade}
%% \cefoot[scrplain-mittig-gerade]{scrheadings-mittig-gerade}
%% \refoot[scrplain-rechts-gerade]{scrheadings-rechts-gerade}
%% \lohead[scrplain-links-ungerade]{scrheadings-links-ungerade}
%% \cohead[scrplain-mittig-ungerade]{scrheadings-mittig-ungerade}
%% \rohead[scrplain-rechts-ungerade]{scrheadings-rechts-ungerade}
%% \lofoot[scrplain-links-ungerade]{scrheadings-links-ungerade}
%% \cofoot[scrplain-mittig-ungerade]{scrheadings-mittig-ungerade}
%% \rofoot[scrplain-rechts-ungerade]{scrheadings-rechts-ungerade}
%% \ihead[scrplain-innen]{scrheadings-innen}
%% \chead[scrplain-zentriert]{scrheadings-zentriert}
%% \ohead[scrplain-außen]{scrheadings-außen}
%% \ifoot[scrplain-innen]{scrheadings-innen}
%% \cfoot[scrplain-zentriert]{scrheadings-zentriert}
%% \ofoot[scrplain-außen]{scrheadings-außen}
% 
% 
%%\usepackage{lastpage} % Stellt 'LastPage' zur Verfuegung
%%\cfoot[Seite \pagemark~von \pageref{LastPage}]{} % Seitenzahl von Anzahl Seiten
% 
%% Angezeigte Abschnitte im Header
%\IfElseChapterDefined{
%   \automark[section]{chapter} %[rechts]{links}
%}{
%   \automark[subsection]{section} %[rechts]{links}
%}
%%
%% Linien (moegliche Kombination mit Breiten)
%\IfChapterDefined{
%   %\setheadtopline{}     % modifiziert die Parameter fuer die Linie ueber dem Seitenkopf
%   \setheadsepline{.4pt}[\color{black}]
%                         % modifiziert die Parameter fuer die Linie zwischen Kopf
%                         % und Textkörper
%   %\setfootsepline{}    % modifiziert die Parameter fuer die Linie zwischen Text
%                         % und Fuß
%   %\setfootbotline{}    % modifiziert die Parameter fuer die Linie unter dem Seitenfuss
%}
% 
%% Groesse des Headers
%%\setlength{\headheight}{1.1\baselineskip}
%% -> eingestellt über Option 'headlines'.
% 
%% Breite von Kopf und Fusszeile einstellen
%% \setheadwidth[Verschiebung]{Breite}
%% \setfootwidth[Verschiebung]{Breite}
%% mögliche Werte
%% paper - die Breite des Papiers
%% page - die Breite der Seite
%% text - die Breite des Textbereichs
%% textwithmarginpar - die Breite des Textbereichs inklusive dem Seitenrand
%% head - die aktuelle Breite des Seitenkopfes
%% foot - die aktuelle Breite des Seitenfusses
%\setheadwidth[0pt]{text}
%\setfootwidth[0pt]{text}

%% Fussnoten =============================================================
% Keine hochgestellten Ziffern in der Fussnote (KOMA-Script-spezifisch):
\deffootnote{1.5em}{1em}{\makebox[1.5em][l]{\thefootnotemark}}
\addtolength{\skip\footins}{\baselineskip} % Abstand Text <-> Fussnote
 
\setlength{\dimen\footins}{10\baselineskip} % Beschraenkt den Platz von Fussnoten auf 10 Zeilen
 
\interfootnotelinepenalty=10000 % Verhindert das Fortsetzen von
                                % Fussnoten auf der gegenüberligenden Seite
                                
%% Schriften (Sections )==================================================
 
%\IfElsePackageLoaded{fourier}{
   \newcommand\SectionFontStyle{\rmfamily}
%}{
%   \newcommand\SectionFontStyle{\sffamily}
%}
 
% -- Koma Schriften --
\IfChapterDefined{%
   \setkomafont{chapter}{\huge\SectionFontStyle}    % Chapter
}
\setkomafont{sectioning}{\SectionFontStyle} %  % Titelzeilen % \bfseries
\setkomafont{pagenumber}{\small\rmfamily}             % Seitenzahl
\setkomafont{pageheadfoot}{\small\rmfamily}        % Kopfzeile
%\setkomafont{pagefoot}{\small\sffamily}        % Kopfzeile
\setkomafont{descriptionlabel}{\itshape}        % Kopfzeile
%
 
\addtokomafont{sectioning}{\color{SectionColor}} % Farbe der Ueberschriften
\IfChapterDefined{%
  \addtokomafont{chapter}{\color{SectionColor}} % Farbe der Ueberschriften
}
\renewcommand*{\raggedsection}{\raggedright} % Titelzeile linksbuendig, haengend

\addtokomafont{section}{\bfseries} % Farbe der Ueberschriften
\addtokomafont{subsection}{\bfseries\itshape} % Farbe der Ueberschriften
\addtokomafont{subsubsection}{\bfseries} % Farbe der Ueberschriften

%% UeberSchriften (Chapter und Sections) =================================
% -- Ueberschriften komlett Umdefinieren --
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/titlesec/titlesec.pdf
\usepackage{titlesec}
 
% -- Section Aussehen veraendern --
% --------------------------------
%% -> Section mit Unterstrich
% \titleformat{\section}
%   [hang]%[frame]display
%   {\usekomafont{sectioning}\Large}
%  {\thesection}
%   {6pt}
%   {}
%   [\titlerule \vspace{0.5\baselineskip}]
% --------------------------------
 
% -- Chapter Aussehen veraendern --
% --------------------------------
%--> Box mit (Kapitel + Nummer ) +  Name
% \titleformat{\chapter}[display]     % {command}[shape]
%   {\usekomafont{chapter}\filcenter} % format
%   {                                 % label
%   {\fcolorbox{black}{shadecolor}{
%   {\huge\chaptertitlename\mbox{\hspace{1mm}}\thechapter}
%   }}}
%   {1pc}                             % sep (from chapternumber)
%   {\vspace{1pc}}                    % {before}[after] (before chaptertitle and after)
% --------------------------------
%--> Kapitel + Nummer + Trennlinie + Name + Trennlinie
%\titleformat{\chapter}[display]  % {command}[shape]
%  {\usekomafont{chapter}\Large \color{black}}  % format
%  {                       % label
%  \LARGE\MakeUppercase{\chaptertitlename} \Huge \thechapter \filright%
%  }%}
%  {1pt}                    % sep (from chapternumber)
%  {\titlerule \vspace{0.9pc} \filright \color{SectionColor}}   % {before}[after] (before chaptertitle and after)
%  [\color{black} \vspace{0.9pc} \filright {\titlerule}]
% --------------------------------
%--> Nummer + Name
\titleformat{\chapter}[hang]{\usekomafont{chapter}\huge\sf\bfseries \color{black}}{\thechapter\filright}{1pc}{}

\titleformat{\section}
  {\usekomafont{section}}{\hspace{-.81cm}{\color{white}\thesection}}{1em}{}
\titleformat{\subsection}
  {\usekomafont{subsection}}{\hspace{-1.005cm}{\color{white}\thesubsection}}{1em}{}
%\titleformat{\subsubsection}
%  {\usekomafont{subsubsection}}{\thesubsubsection}{1em}{}

%% Remove section numbering
%% http://tex.stackexchange.com/questions/80113/hide-section-numbers-but-keep-numbering
%\renewcommand{\thesection}{}
%\renewcommand{\thesubsection}{}
\renewcommand{\thesubsubsection}{}
%\makeatletter
%  \def\@seccntformat#1{\csname #1ignore\expandafter\endcsname\csname the#1\endcsname\quad}
%  \def\@subseccntformat#1{\csname #1ignore\expandafter\endcsname\csname the#1\endcsname\quad}
%  \def\@subsubseccntformat#1{\csname #1ignore\expandafter\endcsname\csname the#1\endcsname\quad}
%  \let\sectionignore\@gobbletwo
%  \let\subsectionignore\@gobblethree
%  \let\subsubsectionignore\@gobblefour
%  \let\latex@numberline\numberline
%  \def\numberline#1{\if\relax#1\relax\else\latex@numberline{#1}\fi}
%\makeatother

%%% Doc: No documentation
% Indent first paragraph after section header
% \usepackage{indentfirst}

%% Add line break after \paragraph{}
  \let\ORGparagraph=\paragraph
  \newcommand{\MYparagraph}[1]{\hfill\vspace{0.1cm}\parbox{\linewidth}{\ORGparagraph{#1}\hfill\vspace{0.1cm}}\reallynopagebreak}
  \let\paragraph=\MYparagraph

\titlespacing\section{0pt}{10pt plus 4pt minus 2pt}{10pt plus 2pt minus 2pt}
\titlespacing\subsection{0pt}{10pt plus 4pt minus 2pt}{10pt plus 2pt minus 2pt}

%% Captions (Schrift, Aussehen) ==========================================
 
% % Folgende Befehle werden durch das Paket caption und subfig ersetzt !
% \setcapindent{1em} % Einrueckung der Beschriftung
%\setkomafont{caption}{\color{black}\small\sffamily\RaggedRight}  % Schrift fuer Caption
% \setkomafont{captionlabel}{\color{black}\small}   % Schrift fuer 'Abbildung' usw.
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/caption/caption.pdf
\usepackage{caption}
% Aussehen der Captions
\captionsetup{
   margin = 0pt,
   font = {bf},
   labelfont = {bf},
   format = plain, % oder 'hang'
   indention = 0em,  % Einruecken der Beschriftung
   labelsep = period, %period, space, quad, newline
   justification = centering, % justified, centering
   singlelinecheck = true, % false (true=bei einer Zeile immer zentrieren)
   position = bottom %top
}

\captionsetup[table]{aboveskip=0pt}
\captionsetup[table]{belowskip=-13pt}

%  \renewcommand{\captionfont}{\emph}
%  \renewcommand{\captionlabelfont}{\emph}
%\setlength{\textfloatsep}{-2.0cm}

%%% Bugfix Workaround
\DeclareCaptionOption{parskip}[]{}
\DeclareCaptionOption{parindent}[]{}
 
 
% Aussehen der Captions fuer subfigures (subfig-Paket)
\IfPackageLoaded{subfig}{
 \captionsetup[subfloat]{%
   margin = 10pt,
   font = {small,rm},
   labelfont = {small,bf},
   format = plain, % oder 'hang'
   indention = 0em,  % Einruecken der Beschriftung
   labelsep = space, %period, space, quad, newline
   justification = RaggedRight, % justified, centering
   singlelinecheck = true, % false (true=bei einer Zeile immer zentrieren)
   position = bottom, %top
   labelformat = parens % simple, empty % Wie die Bezeichnung gesetzt wird
 }
}
 
% Aendern der Bezeichnung fuer Abbildung und Tabelle
% \addto\captionsngerman{% "captionsgerman" fuer alte  Rechschreibung
%   \renewcommand{\figurename}{Abb.}%
%   \renewcommand{\tablename}{Tab.}%
% }
 
% Caption fuer nicht fliessende Umgebungen
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/misc/capt-of.sty
\IfPackageNotLoaded{caption}{
  \usepackage{capt-of} % only load when caption is not loaded. Otherwise compiling will fail.
  %Usage: \captionof{table}[short Titel]{long Titel}
}
%
 
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/mcaption/mcaption.pdf
% Captions in Margins
% \usepackage[
%   top,
%   bottom
% ]{mcaption}
 
%%% Example:
% \begin{figure}
%   \begin{margincap}[short caption]{margin caption}
%     \centering
%     \includegraphics{picture}
%   \end{margincap}
% \end{figure}
 
 
 
% \numberwithin{figure}{chapter} %Befehl zum Kapitelweise Nummerieren der Bilder, setzt `amsmath' vorraus
% \numberwithin{table}{chapter}  %Befehl zum Kapitelweise Nummerieren der Tabellen, setzt `amsmath' vorraus

%%% Inhaltsverzeichnis (Schrift, Aussehen) sowie weitere Verzeichnisse ====
% 
%% http://mirror.ctan.org/macros/latex/contrib/tocvsec2/tocvsec2.pdf
%% Change the tocdepth within document, e.g. adjust for appendix
%\usepackage{tocvsec2}
%  \maxtocdepth{section}
% 
%\setcounter{secnumdepth}{2}    % Abbildungsnummerierung mit groesserer Tiefe
%\setcounter{tocdepth}{1}     % Inhaltsverzeichnis mit groesserer Tiefe
%%
% 
%% Inhalte von List of Figures
%\IfPackageLoaded{subfig}{
%  \setcounter{lofdepth}{1}  %1 = nur figures, 2 = figures + subfigures
%}
% 
%% -------------------------------------------------------
% 
%% Aussehen des Inhaltsverzeichnisses: tocloft
%%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/tocloft/tocloft.pdf
%%% Laden mit Option subfigure in Abhaengigkeit vom Paket subfigure und subfig
%% \IfElsePackageLoaded{subfig}
%%   % IF subfig
%%   {\usepackage[subfigure]{tocloft}}{
%%   % ELSE
%%   \IfElsePackageLoaded{subfigure}
%%     % IF subfigure
%%     {\usepackage[subfigure]{tocloft}}
%%      % Else (No subfig nor subfigure)
%%     {\usepackage{tocloft}}
%%   }
%%
%% %TOCLOFT zerstoert Layout der Ueberschriften von TOC, LOT, LOF
%% \IfPackageLoaded{tocloft}{
%% %
%% %%%% Layout Matthias Pospiech (alles serifenlos)
%% \IfChapterDefined{%
%%   \renewcommand{\cftchappagefont}{\bfseries\sffamily}  % Kapitel Seiten Schrift
%%   \renewcommand{\cftchapfont}{\bfseries\sffamily}      % Kapitel Schrift
%% }
%% \renewcommand{\cftsecpagefont}{\sffamily}            % Section Seiten Schrift
%% \renewcommand{\cftsubsecpagefont}{\sffamily}         % Subsectin Seiten Schrift
%% \renewcommand{\cftsecfont}{\sffamily\bfseries}                % Section Schrift
%% \renewcommand{\cftsubsecfont}{\sffamily}             % Subsection Schrift
%%
%% %%%% Layout aus Typokurz:
%% % % Seitenzahlen direkt hinter TOC-Eintrag:
%% % % Ebene \chapter
%% % \renewcommand{\cftchapleader}{}
%% % \renewcommand{\cftchapafterpnum}{\cftparfillskip}
%% % % Ebene \section
%% % \renewcommand{\cftsecleader}{}
%% % \renewcommand{\cftsecafterpnum}{\cftparfillskip}
%% % % Ebene \subsection
%% % \renewcommand{\cftsubsecleader}{}
%% % \renewcommand{\cftsubsecafterpnum}{\cftparfillskip}
%% % % Abstaende vor Eintraegen im TOC verkleinern
%% % \setlength{\cftbeforesecskip}{.4\baselineskip}
%% % \setlength{\cftbeforesubsecskip}{.1\baselineskip}
%% }
%% % Ende tocloft Einstellungen --------------
% 
%%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/ms/multitoc.dvi
%% TOC in mehreren Spalten setzen
%%\usepackage[toc]{multitoc}
% 
%% -------------------------
%
%
%%% Fix for minitoc to disable warnings related to packages titlesec, hyperref
%\RequirePackage{mtcmess}[2006/03/14]
%  \let\mtcPackageWarningNoLineOLD=\mtcPackageWarningNoLine
%  \renewcommand{\mtcPackageWarningNoLine}[3][]{%
%    \ifthenelse{\equal{#1}{W0099}}{}{ % titlesec
%    \ifthenelse{\equal{#1}{W0030}}{}{ % \part altered due to hyperref
%    \ifthenelse{\equal{#1}{W0023}}{}{ % \part, \chapter change due to hyperref
%    \ifthenelse{\equal{#1}{W0028}}{}{ % \chapter altered due to hyperref
%    \ifthenelse{\equal{#1}{W0024}}{}{ % see log for details
%      \mtcPackageWarningNoLineOLD[#1]{#2}{#3}
%    }}}}}
%  }
% 
%%Schriften fuer Minitoc (Inhaltsverzeichnis vor jedem Kapitel)
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/minitoc/minitoc.pdf
%%% FAQ: http://www.tex.ac.uk/tex-archive/macros/latex/contrib/minitoc/minitoc.bug
%\IfElseChapterDefined{%
% \usepackage{minitoc}
% % \usepackage{mtcoff} %% disables minitoc commands
% 
% \setlength{\mtcindent}{0em} % default: 24pt
% \setcounter{minitocdepth}{1}
% \setlength{\mtcskipamount}{\bigskipamount} % default: \bigskipamount
% \mtcsettitlefont{minitoc}{\normalsize\SectionFontStyle}
% \mtcsetfont{minitoc}{*}{\small\SectionFontStyle} %\color{textcolor}
% \mtcsetfont{minitoc}{section}{\small\SectionFontStyle}
% \mtcsetfont{minitoc}{subsection}{\small\SectionFontStyle}
% \mtcsetfont{minitoc}{subsubsection}{\small\SectionFontStyle} 
% \mtcselectlanguage{german}
% \renewcommand{\beforeminitoc}{\vspace*{0cm}}
% \renewcommand{\afterminitoc}{\vspace*{1cm}\noindent} % Added \noindent as a fix
%}{
% \usepackage{minitoc}
% % \usepackage{mtcoff} %% disables minitoc commands
% 
% \setlength{\stcindent}{0pt} %default
% \setcounter{secttocdepth}{2} %default
% \mtcsettitlefont{secttoc}{\SectionFontStyle}
% \mtcsetfont{secttoc}{*}{\small\SectionFontStyle}%
% \mtcsetfont{secttoc}{subsection}{\small\SectionFontStyle}
% \mtcsetfont{secttoc}{subsubsection}{\small\SectionFontStyle}
%}
%
%\let\mtcPackageWarningNoLine=\mtcPackageWarningNoLineOLD
% 
%% Packages that MUST be loaded before minitoc !
%% hyperref, caption, sectsty, varsects, fncychap, hangcaption, quotchap, romannum, sfheaders, alnumsec, captcont


==> tex/preamble/lists.tex <==
%%% Listen ===============================================================
%
%
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/paralist/paralist.pdf
% \usepackage{paralist}
%
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/enumitem/enumitem.pdf
% Better than 'paralist' and 'enumerate' because it uses a keyvalue interface !
% Do not load together with enumerate.
\IfPackageNotLoaded{enumerate}{
  \usepackage{enumitem} %[shortlabels]
    \setlist{itemsep=0ex plus0.2ex}
    \setenumerate{label=\arabic*.,font=\upshape}
    \setdescription{font=\bfseries\upshape}}
%
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/ncctools/doc/desclist.pdf
% Improved description environment
%\usepackage{declist}

==> tex/preamble/maths.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Math Packages
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
 
% *** Mathematik **************************************
%
% amsmath schon vorher geladen da es vor pst-pdf geladen werden muss
 
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/mh/doc/mathtools.pdf
% Erweitert amsmath und behebt einige Bugs
\usepackage[fixamsmath,disallowspaces]{mathtools}
 
%%% Doc: http://www.ctan.org/info?id=fixmath
% LaTeX's default style of typesetting mathematics does not comply
% with the International Standards ISO31-0:1992 to ISO31-13:1992
% which indicate that uppercase Greek letters always be typset
% upright, as opposed to italic (even though they usually
% represent variables) and allow for typsetting of variables in a
% boldface italic style (even though the required fonts are
% available). This package ensures that uppercase Greek be typeset
% in italic style, that upright $\Delta$ and $\Omega$ symbols are
% available through the commands \upDelta and \upOmega; and
% provides a new math alphabet \mathbold for boldface
% italic letters, including Greek.
% \usepackage{fixmath}
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/onlyamsmath/onlyamsmath.dvi
% Warnt bei Benutzung von Befehlen die mit amsmath inkompatibel sind.
\usepackage[
  all,
  warning
]{onlyamsmath}
 
 
%------------------------------------------------------

 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/misc/braket.sty
\usepackage{braket}  % Quantenmechanik Bracket Schreibweise
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/misc/cancel.sty
%\usepackage{cancel}  % Durchstreichen
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/mh/doc/empheq.pdf
%\usepackage{empheq}  % Hervorheben
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/info/math/voss/mathmode/Mathmode.pdf
%\usepackage{exscale} % Skaliert Mathe-Modus Ausgaben in allen Umgebungen richtig.
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/was/icomma.dtx
% Erlaubt die Benutzung von Kommas im Mathematikmodus
\usepackage{icomma}

%%% Doc: http://www.ctex.org/documents/packages/special/units.pdf
% \usepackage[nice]{nicefrac}

%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/numprint/numprint.pdf
% Modify printing of numbers
%\usepackage{numprint}

%------------------------------------------------------

% For nice arrows over vectors
% \usepackage{esvect}

% Using bold greek letters with \bf
\usepackage{bm}

% Allows arrows in matrices: ldelim, rdelim
\usepackage{bigdelim}

\usepackage[amsmath,thmmarks,hyperref]{ntheorem}
  \theoremstyle{plain}
    %% Update \crefname for cleveref
    \newtheorem{theorem}{Theorem}%[chapter]
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{proposition}[theorem]{Proposition}
    \newtheorem{corollary}[theorem]{Corollary}
    \newtheorem{remark}[theorem]{Remark}
    \newtheorem{definition}[theorem]{Definition}
    \newtheorem{example}[theorem]{Example}
    \newtheorem{conjecture}[theorem]{Conjecture}
  
  %Proof environment
  \theoremstyle{nonumberplain}
    \theoremseparator{.}
    \theoremheaderfont{\bfseries}
    \theorembodyfont{\normalfont}
    \theoremsymbol{$\blacksquare$}
      \RequirePackage{amssymb}
    \newtheorem{proof}{Proof}
    
  %Fix to Definition as math is not in bold in "`Def. 1 ($s$-step)"'
      \makeatletter
    \let\copy@theorem@headerfont=\theorem@headerfont
    \newcommand{\my@theorem@headerfont}{%
        \boldmath\copy@theorem@headerfont\unboldmath
      }
    \let\theorem@headerfont=\my@theorem@headerfont
      \makeatother
    
\usepackage[left]{eurosym}  
\usepackage{siunitx}
    \sisetup{
        color=UnitColor,       %% Prüfen, ob alle Einheiten mit siunitx erstellt wurden; vor Druck auskommentieren
        %forbid-literal-units,
        input-signs={+-<>\leq\geq\pm\mp\approx\sim},
        %per-mode=symbol-or-fraction,
        %retain-explicit-plus,
        %
        load-configurations={
            abbreviations,
        },
        %
        exponent-product=\cdot,
        retain-zero-exponent=true,
        group-digits=integer,
        group-separator={,},
        detect-all=true,
    }
    %\addto\extrasngerman{\sisetup{locale = DE}}
    \DeclareSIUnit\eur{\officialeuro}
    
% Defines \Ordinalstringnum to convert number "2" to literal expression "second"
\usepackage{fmtcount}

% Allows page breaks in mathemaical environments
\allowdisplaybreaks

%------------------------------------------------------

 
%%% Tauschen von Epsilon und andere:
% \let\ORGvarrho=\varrho
% \let\varrho=\rho
% \let\rho=\ORGvarrho
%
\let\ORGvarepsilon=\varepsilon
\let\varepsilon=\epsilon
\let\epsilon=\ORGvarepsilon
%
% \let\ORGvartheta=\vartheta
% \let\vartheta=\theta
% \let\theta=\ORGvartheta
%
% \let\ORGvarphi=\varphi
% \let\varphi=\phi
% \let\phi=\ORGvarphi

==> tex/preamble/misc.tex <==
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/isodate/README
%%% Incompatible: draftcopy
% Tune the output format of dates.
%\usepackage{isodate}

% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% fancy packages
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
 
%%% Doc: No documentation - documented in 'The LaTeX Companion'
% \usepackage{fancybox}   % for shadowbox, ovalbox
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/misc/framed.sty
% \usepackage{framed}
% \renewcommand\FrameCommand{\fcolorbox{black}{shadecolor}}
 
 
%%% Doc: No documentation - documented in 'The LaTeX Companion'
% \usepackage{boxedminipage}

\usepackage[
  footnote,  % Full names appear in the footnote
  smaller,    % Print acronym in smaller fontsize
  printonlyused %
]{acronym}


%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/marginnote/marginnote.pdf
% Summary description: marginnote allows margin note, where \marginpar fails
\usepackage{marginnote}
  \renewcommand*{\marginfont}{\noindent\scriptsize\color{MarginNoteColor}}
  
\usepackage[
    colorinlistoftodos,
%    disable,
    textsize=footnotesize,
        ]{todonotes}
%    \newcommand\todosp[2][]{\todo[color=blue!40,#1]{#2}}

==> tex/preamble/pdf.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% PDF related packages
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/microtype/microtype.pdf
% Optischer Randausgleich mit pdfTeX
\ifpdf
\usepackage[%
  expansion=true, % better typography, but with much larger PDF file.
  protrusion=true
]{microtype}
\fi
 
 
%% Use only instead of hyperref !
% \usepackage[%
%    %ref,     % verweist auf Abschnitte
%    pageref, % verweist auf Seiten
% ]{backref} % Links in BiB back to Citation page/section (can be loaded by hyperref too)
 
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/hyperref/doc/manual.pdf
% Ä=\304; Ö=\326; Ü=\334; ä=\344; ö=\366; ü=\374; ß=\377
\usepackage[
   % Farben fuer die Links
   colorlinks=true,         % Links erhalten Farben statt Kaeten
   urlcolor=LinkColor,    % \href{...}{...} external (URL)
   filecolor=LinkColor,  % \href{...} local file
   linkcolor=LinkColor,  %\ref{...} and \pageref{...}
   menucolor=LinkColor,
   citecolor=LinkColor,
   % Links
   raiselinks=true,       % calculate real height of the link
   breaklinks,              % Links berstehen Zeilenumbruch
   %backref=page,            % Backlinks im Literaturverzeichnis (section, slide, page, none)
   %pagebackref=true,        % Backlinks im Literaturverzeichnis mit Seitenangabe
   verbose,
   hyperindex=true,         % backlinkex index
   linktocpage=true,        % Inhaltsverzeichnis verlinkt Seiten
   hyperfootnotes=false,     % Keine Links auf Fussnoten
   % Bookmarks
   bookmarks=true,          % Erzeugung von Bookmarks fuer PDF-Viewer
   bookmarksopenlevel=1,    % Gliederungstiefe der Bookmarks
   bookmarksopen=false,      % Expandierte Untermenues in Bookmarks
   bookmarksnumbered=true,  % Nummerierung der Bookmarks
   bookmarkstype=toc,       % Art der Verzeichnisses
   % Anchors
   plainpages=false,        % Anchors even on plain pages ?
   pageanchor=true,         % Pages are linkable
   % PDF Informationen
   pdftitle={\thesistitle},             % Titel
   pdfauthor={},            % Autor
   pdfcreator={LaTeX, hyperref, KOMA-Script, pdfeTeX-0.\the\pdftexversion\pdftexrevision}, % Ersteller
   %pdfproducer={pdfeTeX 1.10b-2.1} %Produzent
   pdfstartview=Fit,       % Dokument wird Fit Height geaefnet
   pdffitwindow=true,
   pdfpagemode=UseOutlines, % Bookmarks im Viewer anzeigen
   pdfpagelabels=true,      % set PDF page labels
]{hyperref}
 
\IfPackageLoaded{backref}{
   % % Change Layout of Backref
   \renewcommand*{\backref}[1]{%
     % default interface
     % #1: backref list
     %
     % We want to use the alternative interface,
     % therefore the definition is empty here.
   }%
   \renewcommand*{\backrefalt}[4]{%
     % alternative interface
     % #1: number of distinct back references
     % #2: backref list with distinct entries
     % #3: number of back references including duplicates
     % #4: backref list including duplicates
     \mbox{(Zitiert auf %
     \ifnum#1=1 %
       Seite~%
     \else
       Seiten~%
     \fi
     #2)}%
   }
}
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/oberdiek/hypcap.pdf
% Links auf Gleitumgebungen springen nicht zur Beschriftung,
% sondern zum Anfang der Gleitumgebung
\IfPackageLoaded{hyperref}{%
  \usepackage[figure]{hypcap}
}
 
% Auch Abbildung und nicht nur die Nummer wird zum Link (abgeleitet
% aus Posting von Heiko Oberdiek (d09n5p$9md$1@news.BelWue.DE);
% Verwendung: In \abbvref{label} ist ein Beispiel dargestellt
\providecommand*{\abbvrefname}{Abbildung}
\newcommand*{\abbvref}[1]{%
  \hyperref[#1]{\abbvrefname}\vref{#1}%
}
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/pdfpages/pdfpages.pdf
\usepackage{pdfpages} % Include pages from external PDF documents in LaTeX documents
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/oberdiek/pdflscape.sty
%\usepackage{pdflscape} %  Querformat mit PDF
%
% Pakete Laden die nach Hyperref geladen werden sollen
\LoadPackagesNow % (ltxtable, tabularx)

%% Komprimierung von Bildern in PDF ausschalten
% \ifpdf
%    \pdfcompresslevel=0
% \fi

==> tex/preamble/preamble-commands.tex <==
%%% Packages for LaTeX - programming
%
% Define commands that don't eat spaces.
\usepackage{xspace}
% IfThenElse
\usepackage{ifthen}

%%% Doc: http://www.bakoma-tex.com/doc/latex/oberdiek/ifdraft.pdf
%% Usage: \iffdraft{draft-Modus}{final-Modus}
\usepackage{ifdraft}

%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/oberdiek/ifpdf.sty
% command for testing for pdf-creation
\usepackage{ifpdf} %\ifpdf \else \fi
 
%%% Internal Commands: ----------------------------------------------
\makeatletter
%
\providecommand{\IfPackageLoaded}[2]{\@ifpackageloaded{#1}{#2}{}}
\providecommand{\IfPackageNotLoaded}[2]{\@ifpackageloaded{#1}{}{#2}}
\providecommand{\IfElsePackageLoaded}[3]{\@ifpackageloaded{#1}{#2}{#3}}
%
\newboolean{chapteravailable}%
\setboolean{chapteravailable}{false}%
 
\ifcsname chapter\endcsname
  \setboolean{chapteravailable}{true}%
\else
  \setboolean{chapteravailable}{false}%
\fi
 
 
\providecommand{\IfChapterDefined}[1]{\ifthenelse{\boolean{chapteravailable}}{#1}{}}%
\providecommand{\IfElseChapterDefined}[2]{\ifthenelse{\boolean{chapteravailable}}{#1}{#2}}%
 
\providecommand{\IfDefined}[2]{%
\ifcsname #1\endcsname
   #2 %
\else
     % do nothing
\fi
}
%
% Check for 'draft' mode - commands.
\newcommand{\IfNotDraft}[1]{\ifdraft{}{#1}}
\newcommand{\IfNotDraftElse}[2]{\ifdraft{#2}{#1}}
\newcommand{\IfDraft}[1]{\ifdraft{#1}{}}
 
% Definde frontmatter, mainmatter and backmatter if not defined
\@ifundefined{frontmatter}{%
   \newcommand{\frontmatter}{%
      %In Roemischen Buchstaben nummerieren (i, ii, iii)
      \pagenumbering{roman}
   }
}{}
\@ifundefined{mainmatter}{%
   % scrpage2 benoetigt den folgenden switch
   % wenn \mainmatter definiert ist.
   \newif\if@mainmatter\@mainmattertrue
   \newcommand{\mainmatter}{%
      % -- Seitennummerierung auf Arabische Zahlen zuruecksetzen (1,2,3)
      \pagenumbering{arabic}%
      \setcounter{page}{1}%
   }
}{}
\@ifundefined{backmatter}{%
   \newcommand{\backmatter}{
      %In Roemischen Buchstaben nummerieren (i, ii, iii)
      \pagenumbering{roman}
   }
}{}
 
% Pakete speichern die spaeter geladen werden sollen
\newcommand{\LoadPackagesNow}{}
\newcommand{\LoadPackageLater}[1]{%
   \g@addto@macro{\LoadPackagesNow}{%
      \usepackage{#1}%
   }%
}
 
 
 
\makeatother
%%% ----------------------------------------------------------------

==> tex/preamble/preloaded-packages.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Einige Pakete muessen unbedingt vor allen anderen geladen werden
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
 
%%% Doc: www.cs.brown.edu/system/software/latex/doc/calc.pdf
% Calculation with LaTeX
\usepackage{calc}
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/required/babel/babel.pdf
% Languagesetting
\usepackage[
%  german,
%  ngerman,
%  english,
  american
%  frensh,
]{babel}

%%% Info: http://www.mail-archive.com/ctan-ann@dante.de/msg01512.html
% For adding/using translations like "Theorem/Satz" inside babel, especially for beamer
\usepackage{translator}
 
 
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/required/graphics/grfguide.pdf
% Bilder
\usepackage[%
  %final,
  %draft % do not include images (faster)
]{graphicx}
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/oberdiek/epstopdf.pdf
%% If an eps image is detected, epstopdf is automatically called to convert it to pdf format.
%% Requires: graphicx loaded
\usepackage{epstopdf}
 
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/required/amslatex/math/amsldoc.pdf
% Amsmath - Mathematik Basispaket
%
% fuer pst-pdf displaymath Modus vor pst-pdf benoetigt.
\usepackage[
   centertags, % (default) center tags vertically
   %tbtags,    % 'Top-or-bottom tags': For a split equation, place equation numbers level
               % with the last (resp. first) line, if numbers are on the right (resp. left).
   sumlimits,  %(default) Place the subscripts and superscripts of summation
               % symbols above and below
   %nosumlimits, % Always place the subscripts and superscripts of summation-type
               % symbols to the side, even in displayed equations.
   intlimits,  % Like sumlimits, but for integral symbols.
   %nointlimits, % (default) Opposite of intlimits.
   namelimits, % (default) Like sumlimits, but for certain 'operator names' such as
               % det, inf, lim, max, min, that traditionally have subscripts placed underneath
               % when they occur in a displayed equation.
   %nonamelimits, % Opposite of namelimits.
   %leqno,     % Place equation numbers on the left.
   %reqno,     % Place equation numbers on the right.
   fleqn,     % Position equations at a fixed indent from the left margin rather than
               % centered in the text column.
]{amsmath} %
% eqnarray nicht zusammen mit amsmath benutzen, siehe l2tabu.pdf für Hintergruende.
 
%%% Doc: http://www.ctan.org/tex-archive/macros/latex/contrib/pst-pdf/pst-pdf-DE.pdf
% Used to automatically integrate eps graphics in an pdf document using pdflatex.
% Requires ps4pdf macro !!!
% Download macro from http://www.ctan.org/tex-archive/macros/latex/contrib/pst-pdf/scripts/
%
\usepackage[%
   %active,       % Aktiviert den Extraktionsmodus (DVI-Ausgabe). Die explizite Angabe ist
                  % normalerweise unnötig (Standard im LATEX-Modus).
   %inactive,     % Das Paket wird deaktiviert, Zuätzlich werden die Pakete pstricks und
                  % graphicx geladen
   nopstricks,    % Das Paket pstricks wird nicht geladen.
   %draft,        % Im pdfLATEX-Modus werden aus der Containerdatei eingefügte Grafiken nur
                  % als Rahmen dargestellt.
   %final,        % Im pdfLATEX-Modus werden aus der Containerdatei eingefügte Grafiken
                  % vollständig dargestellt (Standard).
   %tightpage,    % Die Abmessung Grafiken in der Containerdatei entsprechen denen der
                  % zugehörigen TEX-Boxen (Standard).
   %notightpage,  % die Grafiken in der Containerdatei nehmen
                  % mindestens die Größe des gesamten Blattes einnehmen.
   displaymath,   %  Es werden zusätzlich die mathematischen Umgebungen displaymath,
                  % eqnarray und $$ extrahiert und im pdf-Modus als Grafik eingefügt.
]{pst-pdf}
%
% Notwendiger Bugfix für natbib Paket bei Benutzung von pst-pdf (Version <= v1.1o)
\IfPackageLoaded{pst-pdf}{
   \providecommand\makeindex{}
   \providecommand\makeglossary{}
}{}
 
 
%% Doc: ftp://tug.ctan.org/pub/tex-archive/graphics/pstricks/README
% load before graphicx
% \usepackage{pstricks}
% \usepackage{pst-plot, pst-node, pst-coil, pst-eps}
 
% This package implements a workaround for the LaTeX bug that marginpars
% sometimes appear on the wrong margin.
% \usepackage{mparhack}
% in some case this causes an error in the index together with package pdfpages
% the reason is unkown. Therefore I recommend to use the margins of marginnote
  
%% Doc: (inside relsize.sty )
%% ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/misc/relsize.sty
%  Set the font size relative to the current font size
\usepackage{relsize}
 
%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/ms/ragged2e.pdf
% Besserer Flatternsatz (Linksbuendig, statt Blocksatz)
\usepackage{ragged2e}

==> tex/preamble/referencing.tex <==

% Quotes =================================================================
% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/csquotes/csquotes.pdf
% Advanced features for clever quotations
\usepackage[%
   babel=true,            % the style of all quotation marks will be adapted
    german=quotes                 % to the document language as chosen by 'babel'
%   german=guillemets,    % Styles of quotes in each language
%   english=british,
%   french=guillemets
%   style=guillemets
]{csquotes}


  %\MakeAutoQuote{\guillemotright}{\guillemotleft}                % ALT+174, ALT+175
  %\MakeAutoQuote{{\guillemotright}}{{\guillemotleft}}
  %\MakeAutoQuote{»}{«}
 
% All facilities which take a 'cite' argument will not insert
% it directly. They pass it to an auxiliary command called \mkcitation
% which  may be redefined to format the citation.
\renewcommand*{\mkcitation}[1]{{\,}#1}
\renewcommand*{\mkccitation}[1]{ #1}
 
\SetBlockThreshold{2} % Anzahl von Zeilen
 
\newenvironment{myquote}%
  {\begin{quote}\small}%
  {\end{quote}}%
\SetBlockEnvironment{myquote}
%\SetCiteCommand{} % Changes citation command 

\usepackage[%
  %capitalize,
  sort&compress
]{cleveref}
  \crefname{lemma}{lemma}{lemmas}
  \Crefname{lemma}{Lemma}{Lemmas}  
  \crefname{proposition}{proposition}{propositions}
  \Crefname{proposition}{Proposition}{Propositions}
  \crefname{corollary}{corollary}{corollaries}
  \Crefname{corollary}{Corollary}{Corollaries}
  \crefname{remark}{remark}{remarks}
  \Crefname{remark}{Remark}{Remarks}
  \crefname{definition}{definition}{definitions}
  \Crefname{definition}{Definition}{Definitions}
  \crefname{example}{example}{examples}
  \Crefname{example}{Example}{Examples}
  \crefname{conjecture}{conjecture}{conjectures}
  \Crefname{conjecture}{Conjecture}{Conjectures}
  \crefname{proof}{proof}{proofs}
  \Crefname{proof}{Proof}{Proofs}
	\crefname{enumi}{Regel}{Regel}
	\Crefname{enumi}{Regel}{Regel}
	\Crefname{enumi}{Regel}{Regel}
		\IfPackageLoaded{algorithmic}{%
    \crefname{ALC@unique}{step}{steps}
    \Crefname{ALC@unique}{Step}{Steps}
    \crefname{ALC@line}{step}{steps}
    \Crefname{ALC@line}{Step}{Steps}
  }

%%Custom enumerate	
\makeatletter
\newcommand{\labitem}[2]{%
\def\@itemlabel{\textbf{#1}}
\item
\def\@currentlabel{#1}\label{#2}}
\makeatother

%% Adds info boxes on the margin with the name of \label, \ref and \cite
%% Works only in draft mode!
\usepackage[
    notref,
    notcite
  ]{showkeys}
  \providecommand*\showkeyslabelformat[1]{%
\fbox{\tiny\ttfamily#1}}
  
%\usepackage[english]{varioref}                  % cooles Zeug auf S. 72/73
%    \labelformat{table}{\tablename~#1}
%    \labelformat{figure}{\figurename~#1}
%    \labelformat{chapter}{\chaptername~#1}
%    \labelformat{section}{Section~#1}
%    \labelformat{subsection}{Section~#1}
%    \labelformat{subsubsection}{Section~#1}
%    \labelformat{equation}{(#1)}
%%    \labelformat{footnote}{Fußnote~#1\protect\iscurrentchapter{\thechapter}}
%%        \newcommand\iscurrentchapter[1]{%
%%            \ifthenelse{\equal{#1}{\thechapter}}{}{\space in Kapitel~#1}}


==> tex/preamble/symbols.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Symbole
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%
%%% General Doc: http://www.ctan.org/tex-archive/info/symbols/comprehensive/symbols-a4.pdf
%
%% Symbole für Mathematiksatz
%\usepackage{mathrsfs} %% Schreibschriftbuchstaben für den Mathematiksatz (nur Großbuchstaben)
%\usepackage{dsfont}   %% Double Stroke Fonts
%\usepackage[mathcal]{euscript} %% adds euler mathcal font
\usepackage{amssymb}
\usepackage[Symbolsmallscale]{upgreek} % upright symbols from euler package [Euler] or Adobe Symbols [Symbol]
\usepackage[upmu]{gensymb}             % Option upmu
 
%% Allgemeine Symbole
%\usepackage{wasysym}  %% Doc: http://www.ctan.org/tex-archive/macros/latex/contrib/wasysym/wasysym.pdf
%\usepackage{marvosym} %% Symbole aus der marvosym Schrift
\usepackage{pifont}   %% ZapfDingbats

%% http://tex.stackexchange.com/questions/42619/x-mark-to-match-checkmark
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

==> tex/preamble/tables.tex <==
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Tables (Tabular)
% ~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
 
\makeatletter
    \renewcommand{\fps@table}{htbp}         % default {tbp}
\makeatother
 
% Basispaket fuer alle Tabellenfunktionen
% -> wird automatisch durch andere Pakete geladen
% \usepackage{array}
%
% bessere Abstaende innerhalb der Tabelle (Layout))
% -------------------------------------------------
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/booktabs/booktabs.pdf
\usepackage{booktabs}
%
% Farbige Tabellen
% ----------------
% Das Paket colortbl wird inzwischen automatisch durch xcolor geladen
%
% Erweiterte Funktionen innerhalb von Tabellen
% --------------------------------------------
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/multirow/multirow.sty
\usepackage{multirow} % Mehrfachspalten
%
%%% Doc: Documentation inside dtx Package
\usepackage{dcolumn}  % Ausrichtung an Komma oder Punkt
 
%%% Neue Tabellen-Umgebungen:
% ---------------------------
% Spalten automatischer Breite:
%%% Doc: Documentation inside dtx Package
 \usepackage{tabularx}
% -> nach hyperref Laden
% -> wird von ltxtable geladen
% \LoadPackageLater{tabularx}
 
 
% Tabellen ueber mehere Seiten
% ----------------------------
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/carlisle/ltxtable.pdf
% \usepackage{ltxtable} % Longtable + tabularx
                        % (multi-page tables) + (auto-sized columns in a fixed width table)
% -> nach hyperref laden
\LoadPackageLater{ltxtable}
 
 
%%% Doc: ftp://tug.ctan.org/pub/tex-archive/macros/latex/contrib/supertabular/supertabular.pdf
%\usepackage{supertabular}

%    \setlength\extrarowheight{0pt}      % für kleinen space zwischen rows

